Visual Chunking: A List Prediction Framework for Region-Based Object Detection

We consider detecting objects in an image by iteratively selecting from a set of arbitrarily shaped candidate regions. Our generic approach, which we term visual chunking, reasons about the locations of multiple object instances in an image while expressively describing object boundaries. We design an optimization criterion for measuring the performance of a list of such detections as a natural extension to a common per-instance metric. We present an efficient algorithm with provable performance for building a high-quality list of detections from any candidate set of region-based proposals. We also develop a simple class-specific algorithm to generate a candidate region instance in near-linear time in the number of low-level superpixels that outperforms other region generating methods. In order to make predictions on novel images at testing time without access to ground truth, we develop learning approaches to emulate these algorithms' behaviors. We demonstrate that our new approach outperforms sophisticated baselines on benchmark datasets.

==> ExactMaxInterOverUnion_flat.tex <==
%% \documentclass[11pt]{article} % use larger type; default would be 10pt
%% \usepackage[T1]{fontenc}
%% \usepackage[utf8]{inputenc}
%% \usepackage{lmodern}
%% \usepackage{amsmath}
%% \usepackage{listings}
%% \usepackage{graphicx}
%% \usepackage{amsmath}
%% \usepackage{caption}
%% \usepackage{subcaption}
%% \usepackage{graphicx}
%% \usepackage{caption}
%% \usepackage{subcaption}
%% \usepackage[utf8]{inputenc} % set input encoding (not needed with XeLaTeX)
%% \usepackage{algorithm}
%% \usepackage{algorithmic}
%% \usepackage{amsthm}
%% \usepackage{amssymb}

%%% Examples of Article customizations
% These packages are optional, depending whether you want the features they provide.
% See the LaTeX Companion or other references for full information.

%%% PAGE DIMENSIONS
%% \usepackage{geometry} % to change the page dimensions
%% \geometry{a4paper} % or letterpaper (US) or a5paper or....
%% % \geometry{margin=2in} % for example, change the margins to 2 inches all round
%% % \geometry{landscape} % set up the page for landscape
%% %   read geometry.pdf for detailed page layout information

%% \usepackage{graphicx} % support the \includegraphics command and options


%% \title{Exact Maximization of Intersection Over Union}
%% \author{ Jiaji Zhou, Nick Rhinehart, J. Andrew Bagnell, Martial Hebert}

\section{Proof of Optimality} \label{app:emiu}
The output set of superpixels $Z$ is the exact optimum. %First, it is obvious that the optimal solution should not contain superpixels that have zero intersection with ground truth, and should contain all superpixels that are fully inside the ground truth.
Now denote the solution $Z = \{ z_1, z_2, ... , z_m \}$, where it is sorted according to $r_i$. Denote the optimal solution as $Z^* = \{z_1^*,  z_2^*, ... , z_n^*\}$. %We only need to consider the superpixels that is partially overlapping, since both $Z$ and $Z^*$ would contain all superpixels that are fully inside the ground truth. 
Observe that if line 10 is true, i.e., $r_i > R(Z)$, then executing line 11 will always increase $R(Z)$. This is leveraging the fact that superpixels never overlap, and therefore, $R(Z \cup s_i) = \frac{\cap(Z, G) + \Delta_{x_i}}{\cup(Z, G) + \Delta_{y_i}}$. If $r_i = \frac{\Delta_{x_i}}{\Delta_{y_i}} > \frac{\cap(Z, G)}{\cup(Z, G)} $, then $ r_i > R(Z\cup s_i) > R(Z) =  \frac{\cap(Z, G)}{\cup(Z, G)} $. 
We first prove that $Z^* \subseteq Z$ with the following two steps:
\begin{enumerate}
\item$ r(z_i^*) \geq r(z_n^*) > R(Z^*) > R(Z) $, for all $z_i^* \in Z^* $
\item By construction of $Z$ , we have $z_i^* \in Z$. Since if $z_i^*$ is not in $Z$, the algorithm should not stop. 
\end{enumerate}

Next, we prove that $Z \subseteq Z^*$ with the following two steps:
\begin{enumerate}
\item Note that we have already proved that $Z^* \subseteq Z$. Then $z_i = z_i^*$ for $i = 1, ..., n$. Since $z_i$ is in decreasing order of ratio $r_i$, if some $z_i$ ($i = 1, ..., n$) is not in $Z^*$, we can add it into $Z^*$ to increase the value; 
\item For $z_{n+1} ,..., z_{m}$, they cannot exist, which is to say $n = m$. The reason is that $z_{n+1} ,..., z_{m}$ would always increase $R(Z)$ by the construction of  algorithm, which contradicts with the assumption that $Z^*$ is the optimum 
\end{enumerate}


\section{Error Analysis for Grower}
\subsection{Multiplicative and Additive Bound for Grower}
Let $\alpha_1 \geq \alpha_2 \geq \cdots \geq \alpha_N $, let the optimal solution for I/U be the first $k$ superpixels; Suppose the regressor makes bounded uniform error $\epsilon$, i.e., $|\hat{\alpha}_i - \alpha_i| < \epsilon$. Further, let $M$ be the largest number such that: $\alpha_j \geq \alpha_k - 2\epsilon$ for $j = 1 ,..., M$. 

If the regressor makes bounded uniform error $\epsilon$, then the worst case would be: it underestimates $\alpha_1 ,..., \alpha_k$ by $\epsilon$ and overestimates $\alpha_{k+1} ,..., \alpha_M $ by $\epsilon$. Therefore, some of the elements in $\alpha_{k+1} ,..., \alpha_M $ would rank higher than $\alpha_1 ,..., \alpha_k$.  
Denote $Z$ as the best solution among the chain of sets induced by the ranking output of the regressor.  We proceed with analyzing the worse case performance under the bounded uniform error assumption. 
\begin{align}
  f(Z) & \geq f(\{\alpha_1, ..., \alpha_M \}) = \frac{\sum_{i=1}^M{Area_i \alpha_i}}{Area_G + \sum_{i=1}^M{Area_i (1-\alpha_i)}} \\
  & = \frac{\sum_{i=1}^k{Area_i \alpha_i} + \sum_{j=k+1}^M{Area_j \alpha_j} }{Area_G + \sum_{i=1}^k{Area_i (1-\alpha_i)} + \sum_{j=k+1}^M{Area_j (1-\alpha_j)}} \\
  & \geq \min\{ \frac{\sum_{i=1}^k{Area_i \alpha_i}}{Area_G + \sum_{i=1}^k{Area_i (1-\alpha_i)}},  \frac{\sum_{i=k+1}^M{Area_i \alpha_i}}{\sum_{i=k+1}^M{Area_i (1-\alpha_i)}} \} \\
  & = \min\{ f(OPT), \frac{\sum_{i=k+1}^M{Area_i \alpha_i}}{\sum_{i=k+1}^M{Area_i (1-\alpha_i)}}  \} \\
  & = \frac{\sum_{i=k+1}^M{Area_i \alpha_i}}{\sum_{i=k+1}^M{Area_i (1-\alpha_i)}} \\
 &  \geq \frac{\sum_{i=k+1}^M{Area_i (\alpha_k - 2\epsilon) }}{\sum_{i=k+1}^M{Area_i (1-(\alpha_k -2\epsilon) )}} \\
 %& = \frac{ (\alpha_k - 2\epsilon)\sum_{i=k+1}^M{Area_i}} {(1-\alpha_k + 2\epsilon ) \sum_{i=k+1}^M{Area_i} }
 & = \frac{ (\alpha_k - 2\epsilon)} {(1-\alpha_k + 2\epsilon )  }  \label{boundalpha} 
\end{align}
Since $r_k = \frac{\alpha_k}{1 - \alpha_k} \geq f(OPT)$, we would have $ 1 - \alpha_k \leq \frac{\alpha_k}{f(OPT)}$, therefore we can proceed as follows:
\begin{align}
f(Z) \geq \frac{ (\alpha_k - 2\epsilon)} {(1-\alpha_k + 2\epsilon )  } \\
\geq \frac{f(OPT)(\alpha_k - 2\epsilon)}{\alpha_k + 2\epsilon f(OPT)}
\end{align}
Next, we bound the ratio of $f(Z)$ over $f(OPT)$:
\begin{align}
\frac{f(Z)} {f(OPT)} & \geq \frac{\alpha_k - 2\epsilon}{\alpha_k + 2\epsilon f(OPT)} \\
&= \frac{\alpha_k + 2\epsilon f(OPT)- 2\epsilon(1 + f(OPT))}{\alpha_k + 2\epsilon f(OPT)}\\
&= 1 - \frac{ 2\epsilon(1 + f(OPT))}{\alpha_k + 2\epsilon f(OPT)} \\
& \geq 1 -  \frac{ 2(1 + f(OPT))}{\alpha_k} \epsilon\\ 
& \geq 1 - \frac{4}{\alpha_k} \epsilon  \label {beforerelaxfracalpha} \\
& \geq 1 - \frac{4}{(1/f(OPT) + 1)} \epsilon \label{afterrelaxfracalpha}
\end{align}

From \eqref{beforerelaxfracalpha} to \eqref{afterrelaxfracalpha}, we are using the fact that $\frac{1}{r_k} = \frac {1}{\alpha_k} - 1 \leq \frac{1}{f(OPT)}$. 

We can proceed to have an additive bound:

\begin{align}
f(OPT) - f(Z) &\leq \frac{4f(OPT)} {1/f(OPT) + 1} \epsilon \label{beforerelaxf(OPT)}  \\ 
                  & \leq 2\epsilon \label{afterrelaxf(OPT)}
\end{align}
From \eqref{beforerelaxf(OPT)} to \eqref{afterrelaxf(OPT)}, we are using the fact that $f(OPT)\leq 1$

%\input{old_additive_bound}


\subsubsection{The Expectation Case }
A more natural assumption is to assume an expected square error $\epsilon$ over the distribution $P$ of all superpixels. Denote $\delta = \E_{i \sim P} (\hat{r_i} - r_i)^2$, we would have that for each image $j$, the expected uniform error bound $\E[\epsilon^j]$ satisfies:
\begin{align}
 \E[\epsilon^j] & = \E [ \max_i | \epsilon_i | ] \\
  & = \E [ ( \max_i \epsilon_i^2 )^{\frac{1}{2}} ] \\
 & \leq \E [ ( \sum_i \epsilon_i^2 )^{\frac{1}{2}} ]  \\ 
&\leq \E[ n \epsilon^2 ]^{1/2}  \textrm{(by Jensen's inequality and the fact that $\sqrt{x}$ is concave) ~} \\
&\leq \sqrt{n \delta}
\end{align}
Along with the additive bound above, we have the following error bound theorem



%% \bibliography{references}
%% \bibliographystyle{plain}
%% \end{document}


==> OuterLoopInference_flat.tex <==
\begin{algorithm} 
\caption{Chunk List Prediction Inference} \label{alg:outer_loop_greedy_inference}
\begin{small}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Image $I$, Trained List Predictor $Z$, Number of predictions $R$, optional threshold, $t$
\STATE \textbf{Ouput:} List of chunk predictions $L_g$

\STATE $C = \mathtt{[]}$
\FOR{$r=0$ \textbf{to} $R$}
\STATE $(C_r, s) = Z.\mathtt{predict}(I, C)$
\IF{$s < t$}
\STATE \textbf{return} $C$
\ENDIF
\STATE $L_g = \left[L_g, C_r\right]$
\ENDFOR
\STATE \textbf{return} $C$

\end{algorithmic}
\end{small}
\end{algorithm}



==> OuterLoopSCP_flat.tex <==
We begin by defining a natural scoring function to evaluate any input list of chunks given ground-truth on the pixels corresponding to objects of interest in a scene. We provide an efficient greedy algorithm that is guaranteed to optimize this metric to within a constant factor given access to ground ground truth and this arbitrary list of (potentially overlapping) candidate chunks (Section \ref{sec:list_gt}). 

Of course, at testing time there is no access to the ground truth of where objects are in the scene. Our approach then, following recent work in structured prediction \cite{ross2013learning, daume2009search}, is to learn to mimic the sequential greedy strategy. The result is a simple predictor that takes a candidate set of chunks, and iteratively grows a list of chunks that likely correspond to separate objects in the scene.

Note that we do not place assumption on the given candidate set of chunks: the list predictor is agnostic to the way the candidate set of chunks was generated; it merely chooses the best one  in the set. Such a set can be heuristically generated in many ways, \emph{e.g.}, those created from the baseline approaches to visual chunking we describe above. In section \ref{sec:chunk_grow}, however, we provide an algorithm designed to generate a candidate set that contains good chunks based on a fixed superpixel-based segmentation.

\subsubsection{Objective Function and Greedy Optimization} \label{sec:list_gt}
Given an image with ground truth entities set $G$ and candidate chunks set $C$, our goal is to sequentially build a list of chunks out of $C$ so as to maximize the sum of intersection over union with respect to ground truth entities.  Define $L = \{c_1, c_2, \dots, c_{|L|} \}$ as a list of chunks with $c_i \in C$
 and $\tilde{G} = \{ \tilde{g}_1, \tilde{g}_2, \dots, \tilde{g}_{|L|}  \}$ with $\tilde{g}_i$ either be a real ground truth entity $g_i$ from $G$ or a ``dummy" ground truth entity which gives zero I/U score.  

Each $c_i$ is associated with at most one real ground truth entity $g_i$ , and each $g_i$ is associated with at most one $c_i$. Chunks that do not overlap ground truth objects have zero score. ``Dummy" ground truth is used as a notational convenience, to handle cases when the length of predicted list is larger the total number of ground truth entities, where some chunks in $L$ would otherwise have no ground truth entity to associate with. It can be seen that each different permutation of $\tilde{G} $ corresponds to different associations between predicted chunks in list $L$ and the ground truth entities in $G$.
For any given list $L$ and $\tilde{G}$, let $h(L, \tilde{G})$ be the sum of I/U sores of the corresponding associations:
\begin{equation*}
    h(L, \tilde{G}) = \sum_{i=1}^{|L|}\|\frac{c_i\cap{\tilde{g}_i}}{c_i\cup{\tilde{g}_i}} \|
\end{equation*}
We define the score of the list, $f(L)$, to be the sum of I/U scores for the optimum association with ground truth entities, i.e., $f(L) = \{\max_{\tilde{G}} h(L, \tilde{G}) \} $.   We can express our goal in terms of maximizing the following objective function $f$:
\begin{equation}
	 \max_{L} f(L) = \max_{L}\{\max_{\tilde{G}} \sum_{i=1}^{|L|} \frac{\|c_i\cap{\tilde{g}_i}\|}{\|c_i\cup{\tilde{g}_i\|}} \} \label{list_obj_func} .
\end{equation}
%$f(L) = \{\max_{\tilde{G}} \sum_{i=1}^m \frac{c_i\cap{\tilde{g}_i}}{c_i\cup{\tilde{g}_i}} \} $ is the sum of intersection over union of each chunk-ground truth entity association over the best permutation $\tilde{G}$.  
This scoring metric, which is a natural generalization of the Intersection over Union metric common in segmentation and single entity detection \cite{Everingham10, arbelaez2012semantic}, encourages 
lists of a fixed length that contain chunks that are relevant and diverse in covering multiple ground truth entities. 
Unfortunately, the metric as written down does not possess the clear combinatorial structure like modularity or submodularity 
that would enable us to easily optimize it.

Interestingly, however, Problem~(\ref{list_obj_func}) can be cast as an equivalent maximum weighted bi-partite graph matching problem. This can be shown to be a  simple modular (i.e. additive) maximization problem under matroid constraints~\cite{lin2011word} and the solution $L^{gr}$ returned by a simple greedy algorithm is guaranteed to be near-optimal~\cite{fisher1978analysis}. The greedy algorithm then constructs a list $L^{gr}$ using the corresponding $\tilde{G}^{gr}$ as follows:
\begin{align*}
(c_{1}^{gr}, \tilde{g}_{1}^{gr})  & =  \argmax_{c \in C, g\in G}\frac{\|c \cap g\|}{\|c \cup g\|}, \\ 
 (c_{2}^{gr}, \tilde{g}_{2}^{gr}) & =  \argmax_{c \in C \setminus{c_1^{gr}}, g \in G \setminus{\tilde{g}_{1}^{gr}} }\frac{\|c \cap g\|}{\|c \cup g\|},  \\
 \vdots\\
 (c_{k}^{gr}, \tilde{g}_{k}^{gr}) & =  \argmax_{c\in C \setminus {\{c_1^{gr} \dots c_{k-1}^{gr}\}}, g \in G \setminus {\{\tilde{g}_1^{gr} \dots \tilde{g}_{k-1}^{gr}\}}}\frac{\|c \cap g\|}{\|c \cup g\|} 
\end{align*}

Critically, the greedy algorithm is recursive, meaning longer lists of predictions always include shorter lists, and is within a constant factor of optimal:
\begin{thmNearOptGreedyDef}
Let $L_{i}^{gr}$, $ \tilde{G}_{i}^{gr}$ denote the list of the first $i$ elements in $L^{gr}$ and $\tilde{G}^{gr}$ respectively, and $L_{i}^*$ be the optimal solution of Problem (\ref{list_obj_func}) among size-$i$ lists, we have that:
\begin{displaymath}  
f(L_{i}^{gr}) \geq h(L_{i}^{gr}, \tilde{G}_{i}^{gr}) \geq \frac{1}{3} f(L_{i}^*)
\end{displaymath}
for $i = 1,...,|L^{gr}|$.
\end{thmNearOptGreedyDef}
See appendix for proof of Theorem \thmNearOptGreedy. 
The implication of Theorem \thmNearOptGreedy is that if we are given a budget $|L|$ to build the list, then each $L_{i}^{gr}$ is also a near optimal list among all lists of budget $i$, for $i=1, \dots, |L|$. This is an important property for producing good predictions earlier in the list and for producing the list of chunks rapidly.
Moreover, this is the worst case bound, and in our empirical experiments, the quality of solutions, based upon the candidate set of chunks generated by the growing algorithm in \ref{Grower}, are usually much better than this bound suggests. Intuitively, if the candidate set is of high quality that each ground truth is provided with sufficient good chunks to associate with, rather than sharing, then the empirical performance of the greedy algorithn is close to optimal.

\subsubsection{List Prediction Learning} \label{sec:list_learning}
 
In essence, the greedy strategy is a sequential list prediction process, where at each round, it maximizes the marginal benefit given the previous list of predictions and ground truth association. Intuitively, maximization of the marginal benefit at each position of the list yields chunks that have high intersection over union with ground truth entities and minimal overlap with each other. 

%We would like to train a predictor to imitate the above sequential greedy process. To be concrete, at each round $r$, the predictor should rank each of unassigned candidate chunk $c$ based on a score $h(c) = \max_{g \in G_{re}} \frac{c \cap g}{c \cup g}$, where $G_{re}$ is the remaining  ground truth entities.

We adopt an approach following that of \cite{ross2013learning, ross2011learning} where we train a learning algorithm to mimic this greedy procedure. The  training procedure as illustrated in Algorithm \ref{outerloop_training}.  We denote by $\Phi(c, L)$ the feature vector that represents the interaction between each input chunk $c$, any given list $L$ and their interactions. This includes features measuring the affinity or similarity between $c$ and elements in $L$, and intuitively, a high affinity feature implies that appending $c$ to $L$ is less preferred as it is similar to exising items in the list. We discuss the features design in \ref{sec:features}.
We denote by $\tilde{G}^{gr}(L)$  the corresponding greedy association for any list $L$,  and we define the greedy marginal benefit of adding chunk $c$ to $L$ be $y(c, L) = h(L\oplus c, \tilde{G}^{gr}(L\oplus c)) - h(L, \tilde{G}^{gr}(L)) $.

\begin{algorithm}[!t] 
\caption{List Predictor Training Algorithm Using DAgger}
\label{outerloop_training}
\begin{algorithmic}
\STATE \textbf{Input:}  $T$ images, each with candidate chunk set $C^t$ and $G^t$, number of training iterations $R$, list size $k$  
\STATE \textbf{Output:} A trained list predictor/predictor $\pi$
\STATE Initialize $D \gets \emptyset$
\STATE Set $\pi_0$ to be the greedy oracle predictor 
\FOR{$i = 1$ \textbf{to} $R$ }
	\FOR{$t = 1$ \textbf{to} $T$}
	\STATE $L^t = $\textrm{Predict}$(C^t, \pi_{i-1}, k)$.
	\STATE Get dataset $D^t_i = \{ X_{j=1}^{k}, Y_{j=1}^{k} \}$ using $L^t$, $C^t$ and $G^t$.
	\STATE $D \gets D \cup D^t_i$.
	\ENDFOR
	\STATE Train $\pi_{i}$ on D
\ENDFOR
\STATE Return $\pi_{R}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!t] 
\SetAlgorithmName{Procedure}{procedure}{List of procedure}
%\caption{Predict$(C, \pi_{i-1}, k)$}
%\begin{small}
\begin{algorithmic}
\STATE \textbf{Procedure:} Predict$(C, \pi_{i-1}, k)$ 
\STATE \textbf{Input:} Candidate chunk set $C$, List Predictor $\pi$, list size $k$ 
\STATE \textbf{Output:} A list $L$ of chunks
\STATE Initialize $L$ = \{ \}.
\FOR{$ i = 1$ \textbf{to} $k$}
	\STATE $c_i = \argmax_{c \in C}\pi(\Phi(c, L ))$
	\STATE $L = L \oplus c_i$
\ENDFOR
\STATE Return L
\end{algorithmic}
%\end{small}
\end{algorithm}

   The DAgger training mechanism is beneficial in that the policy iteration collects data aimed to improve its own performance. See \cite{ross2010reduction} for more details.  
  %This training algorithm is iterative and begins by generating data assuming all earlier positions in the list were filled in using the greedy predictor with oracle access to the ground truth data. After the first iteration, however, it is learning to correct it's own mistakes: i.e. it will learn that earlier predictions maybe imperfect and adjust the lists it creates.
  
  At each iteration, the predictor from the last iteration loops over every training image $t$ and generates a list prediction $L^t$, as illustrated in $\mathrm{Predict()}$ procedure. As this list is built, we record the marginal benefit of adding other possible elements. Consider the case where the predictor initially chooses a chunk that covers the entire image, in which there is a single ground truth entity. We can improve the list by appending to it a chunk that has a higher I/U score with the entity, and then updating the association between chunks and entities.
 
The algorithm then collects target data $D^t_i = \{ X_{j=1}^{k}, Y_{j=1}^{k} \}$ consisting of features and the true marginal benefits measure on training data using $L^t$, $C^t$ and $G^t$, where: 
	\begin{enumerate}
	\item $ X_{j=1}^{k}$ is a collection of feature matrices whose element $X_j$ of size $|C_t| \times d$ is formed by stacking the $d$-dimenional feature vectors $\Phi(c, L_j)$, where $c\in C^t$ and $L_j$ is the list of the first $j$ elements in $L$
	\item $Y_{j=1}^k$  is a collection of greedy marginal benefit vectors whose  element $Y_j$ of length $|C_t|$ records $y(c, L_j)$ for each chunk $c\in C^t$
	\end{enumerate}
Each $D^t_i$ is appended to the old training data collection from last iteration to form a larger training dataset $D$, before being utilized to train a regression that predicts benefits. 

Given a new image with a set of candidate chunks, we can call  $\mathrm{Predict()}$ procedure to produce a list of specified length. 


==> OuterLoopTrainingAlgorithm_flat.tex <==
%% \begin{algorithm}[!ht] 
%% \caption{Chunk List Prediction Training \label{alg:ChunkListPrediction}}
%% \begin{small}
%% \begin{algorithmic}[1]

%% %\STATE \textbf{Input:} Sets of sets of chunks $C = \{C_0 = \{C_{00}, C_{01}, \dots, C_{0N_0}\}, \dots, C_M = \{C_{M0}, \dots, C_{MN_M}\}\}$  \\ A set of ground truth entities $G = \{G_0, \dots, G_M\}$ \\ Number of iterations, $I$ \\ Number of rounds, $R$.
%% \STATE \textbf{Input:} A set of images: $I = \{I_0, \dots, I_T\}$, sets of chunks for each image: $C = \{C_0, \dots, C_T\}$, sets of ground truth entities for each image: $G = \{G_0, \dots, G_T\}$. \\ Number of SCP iterations $S$ \\ Number of rounds, $R$.
%% \STATE \textbf{Output:} A single predictor, $P$
%% \STATE $X = [], Y = []$
%% \FOR{$s=0$ \textbf{to} $S$}
%% \FOR{$i=0$ \textbf{to} $T$}
%% \FOR{$r=0$ \textbf{to} $R$}
%% \IF {$|G_i| < r$} 
%% \STATE continue \COMMENT{No GT entities left for image $I_i$}
%% \ENDIF
%% \STATE $h_{max} = 0$
%% \FOR{$c=0$ \textbf{to} $|C_t|$}
%% \STATE $y = h(c)$
%% \IF {$y > h_{max}$}
%% \STATE $h_{max} = y$, $best\mathunderscore chunk = c$
%% \ENDIF
%% \STATE $Y = [Y, y]$
%% \STATE $X = [X, F(c)]$
%% \ENDFOR
%% \STATE $L_i = [L_i, best\mathunderscore chunk]$
%% \ENDFOR
%% \ENDFOR
%% \ENDFOR
%% \end{algorithmic}
%% \end{small}
%% \end{algorithm}



==> Outerloop_Training_flat.tex <==
\begin{algorithm}[!ht] 
\caption{List Predictor Training Algorithm Using DAGGER}
\label{outerloop_training}
%\begin{small}
\begin{algorithmic}
\STATE \textbf{Input:}  $T$ images, each with candidate chunk set $C^t$ and $G^t$, number of training iterations $R$, list size $k$  
\STATE \textbf{Output:} A trained list predictor/policy $\pi$
\STATE Initialize $D \gets \emptyset$
\STATE Set $\pi_0$ to be the greedy oracle policy 
\FOR{$i = 1$ \textbf{to} $R$ }
	\FOR{$t = 1$ \textbf{to} $T$}
	\STATE $L^t = $\textrm{Predict}$(C^t, \pi_{i-1}, k)$.
	\STATE Get feature-marginal score pair dataset $D^t_i = \{ X^t, Y^t \}$ using $L^t$, $C^t$ and $G^t$ 
	\STATE $D \gets D \cup D^t_i$.
	\ENDFOR
	\STATE Train $\pi_{i}$ on D
\ENDFOR
\STATE Return $\pi_{R}$
\end{algorithmic}
%\end{small}
\end{algorithm}

\begin{algorithm}[!ht] 
\SetAlgorithmName{Procedure}{procedure}{List of procedure}
%\caption{Predict$(C, \pi_{i-1}, k)$}
%\begin{small}
\begin{algorithmic}
\STATE \textbf{Procedure:} Predict$(C, \pi_{i-1}, k)$ 
\STATE \textbf{Input:} Candidate chunk set $C$, List Predictor $\pi$, list size $k$ 
\STATE \textbf{Output:} A list $L$ of chunks
\STATE Initialize $L$ = \{ \}.
\FOR{$ i = 1$ \textbf{to} $k$}
	\STATE $c_i = \argmax_{c \in C}\pi(\Phi(c_i, L ))$
	\STATE $L = L \oplus c_i$
\ENDFOR
\STATE Return L
\end{algorithmic}
%\end{small}
\end{algorithm}


==> acknowledgements_flat.tex <==
We would like to thank Daniel Munoz for access to scene parsing system we used in this work.


==> approach_old_flat.tex <==
%%To predict a list of objects, we must have a set of candidate chunks: candidate object detections.  If computational feasability were not an issue, we would propose to our predictor the set of all possible chunks: all possible unions of 1 or more superpixels in an image. The number of chunks is combinatorial, and thus infeasible to compute. Instead, we must create a subset of feasible chunks. Thus, we break the list prediction into two steps:

\input{growing_fig.tex}

To motivate our approach of visual chunking, we first introduce three simple methods leveraging existing bounding box detections\cite{felzenszwalb2010object, dalal2005histograms} and/or superpixel-wise semantic labeling algorithm\cite{munoz-eccv-10}, all of which will serve as our baseline models:

\begin{enumerate}
\item Use bounding box detection algorithm output.
\item Connect an edge between any two adjacent pixels of same semantic labeling output, and treat each connected components as detection output. 
\item Use the intersections of connected components found above and bounding box detections.   
\end{enumerate} 
The drawback of merely using bounding boxes is obvious: rectangular detection boxes violates the fact that object shapes are usually irregular. As for connected components method based on semantic labelling output, one would imagine that, with good semantic labelling output, it would produce reasonable result when objects are well separated in the image. However, when objects are cluttered, e.g., cars on the street, semantic labeling algorithm will not separate them, but rather labels them as one big area [Need figures?]. Further intersection with detection boxes would help, but suffers from compounding errors from both sides. %The errors bounding box detection such as imposing fixed aspect ratios and non-max suppression post processing   
We therefore need a systematic approach to produce region-based detection for cluttered scenarios. We consider  a chunk as a set of superpixels and decompose the task into two parts:
\begin{enumerate}
\item Given an arbitrary set of chunks, we formulate the problem as an optimal matching problem and make a reduction to constrained modular maximization problem where efficient greedy algorithm gives suboptimal guarantee. As for learning, we utilize the contextual list prediction method to imitate the greedy algorithm that enables us to select $k$ chunks that are both relevant and diverse. ????????[How do we say the suboptimal guarantee here? There is no no-regret reduction for this now]  
\item Given the segmentation algorithm, we propose a chunk growing algorithm that is guaranted to contain the optimal chunk given access to ground truth entity at training time. The algorithm runs efficiently in \BigO{n\log n} time, where $n$ is the number of superpixels. We also propose a learning algorithm that enables us to grow chunks effciently at prediction time when we do not know the ground truth entities. 
\end{enumerate}  

%\begin{enumerate}
%\item{Produce a pool of candidate chunks}
%\item{Iteratively select chunks from the candidate pool to build a list of detections}
%\end{enumerate}

%Na\"{\i}ve heurisics for adding to this pool of feasible chunks were investigated, and found to be ineffective and not expressive enough to capture the wide variability of ground-truth entity shapes and scales. Therefore, we designed a learning procedure to build diverse pools of chunks. We also treat this procedure as a list prediction problem, except we desire to product many candidate lists. We iteratively add superpixels to each candidate list; visually, this can be interpreted as ``growing'' chunks.  
\subsection{Chunk Prediction}

\input{OuterLoopSCP}

\subsection{Chunk Growing}

\input{MaxIU}



==> experiments_cur_flat.tex <==
\newlength{\lmsunwidth}
\setlength{\lmsunwidth}{.48\textwidth}


We describe our experiments and predictor features in the next two sections, and discuss the results of each experiment in their respective captions.

\subsection{Datasets and baseline algorithms}
We perform experiments on imagery from 3 different datasets. We refine the Stanford Background Dataset \cite{GouFulKol09} labeling to include a \texttt{vehicle} class with instance labeling. We also perform experiments on PASCAL VOC 2012 (Figure~\ref{fig:voc2012} and Tables~\ref{tab:sum_iu_sbd} and \ref{tab:voc2012}). This dataset possesses relatively few images containing adjacent and/or overlapping instances of the same class. Therefore, we created a subset of the LM+Sun dataset \cite{tighe2010superparsing} of images containing at least 2 adjacent cars, consisting of 1,042 images.



\begin{figure}[t]
        %% \tiny
        \centering
    %% \subfloat[][\tiny LM+Sun Adjacent Cars candidate quality. A previously proposed metric for candidate pool quality is Average Best Overlap (ABO), in which the best overlapping candidate for every ground truth object is computed, and then averaged across the dataset. We find that our grown chunks generally outperform the Selective Search and SCALPEL methods ]{
\vspace{-10pt}
        \begin{minipage}[t]{
            \lmsunwidth}    
\vspace{0pt}   
            \centering
            %% \includegraphics[width=\textwidth]{abo/abo_all_methods.png}
            \includegraphics[width=\textwidth]{abo/abo2_crop.png}
    %% \caption{\tiny LM+Sun Adjacent Cars candidate quality, measured by Average Best Overlap (ABO). We find that our grown chunks generally outperform the Selective Search and SCALPEL methods} \label{fig:lmsun_abo_and_lp}
    \caption{LM+Sun Adjacent Cars candidate quality, measured by Average Best Overlap (ABO). We find that our grown chunks generally outperform the Selective Search and SCALPEL methods. On average, SCALPEL generated $893$ regions per image, Selective Search generated $552$ regions per image, SP~$\cap$~DPM generated 8 chunks per image, and our grower generated $705$ chunks per image.} \label{fig:lmsun_abo_and_lp}
    \end{minipage}
\end{figure}

We evaluate three methods\footnote{
We use the semantic labeling algorithm
of \cite{munoz-eccv-10} and the DPM detection method of
\cite{felzenszwalb2010object} for bounding box output, with the
default SVM threshold, and NMS threshold of $0.5$. To generate the superpixels, we use the segmentation algorithm of \cite{felzenszwalb2004efficient}. For each experiment, separate
semantic labeling systems and chunk growers were trained. 
} leveraging existing bounding box detections and superpixel-wise semantic labeling algorithm, all of which serve as our baseline systems for building lists of predictions: \textbf{1)} Bounding box detector output after NMS filtering \textbf{2)} Connected components of scene parsing (``SP'') / semantic labeling \textbf{3)} A combination of \textbf{1)} and \textbf{2)}: intersection of connected components with bounding boxes, which creates chunks for every bounding box by extracting the labeled region inside (``SP $\cap$ DPM''). The third baseline is intended to capitalize on desirable properties of each component while avoiding their less desirable properties: boxes usually violate the object boundaries, and semantic labeling does not separate adjacent instances. The downside to this baseline is that it can suffer from
compounding both detector and scene parsing  errors. See Figure~\ref{fig:us_vs_them_all} for a visual comparison.
%% \footnote{\footnotesize Note that this baseline is actually quite sophisticated, as it
  %% leverages state-of-the-art methods in both detection and semantic
  %% parsing. Its major performance shortcoming is in handling occluding instances.}

%% \footnote{We note that the final baseline in particular is actually quite sophisticated: it leverages complementary methods that are close to the state-of-the-art in both detection and semantic parsing. In particular, the only images where one can attempt to compete with such a baseline is on objects that are in close proximity, a point we highlight further in our experimental section.}
%% \begin{figure}[h!]
%%         \centering
%%         \subfloat[][1-instance images]{\includegraphics[width=.3\textwidth]{img/fixed_vehicle/sum_iu_During_Testing_3-6-16-47_1prediction_budget.png}}
%%         \subfloat[][2-instance images]{\includegraphics[width=.3\textwidth]{img/fixed_vehicle/sum_iu_During_Testing_3-6-16-47_2prediction_budget.png}}
%%         \subfloat[][3-instance images]{\includegraphics[width=.3\textwidth]{img/fixed_vehicle/sum_iu_During_Testing_3-6-16-47_3prediction_budget.png}}\\
%%         \vspace{-10pt}
%%         \subfloat[][1-instance images]{\includegraphics[width=.3\textwidth]{img/fixed_voc_person/sum_iu_During_Testing_3-6-16-49_1prediction_budget.png}}
%%         \subfloat[][2-instance images]{\includegraphics[width=.3\textwidth]{img/fixed_voc_person/sum_iu_During_Testing_3-6-16-49_2prediction_budget.png}}
%%         \subfloat[][3-instance images]{\includegraphics[width=.3\textwidth]{img/fixed_voc_person/sum_iu_During_Testing_3-6-16-49_3prediction_budget.png}}\\
%% \subfloat[][Legend]{\includegraphics[width=.3\textwidth]{img/sum_iu_instance_legend_fixed.png}}       
%% \caption{These experiments are similar to those displayed in
%%   Figure~\ref{fig:sum_iu_all}. The top row corresponds to the SBD
%%   \texttt{vehicle} class, and the bottom row corresponds to the PASCAL
%%   VOC 2012 \texttt{person} class. For each graph, a subset of the test
%%   data is taken corresponding to the images that contain exactly $m$
%%   ground-truth instances. The ``ideal'' I/U score line (black) is the
%%   minimum of the number of predictions made and the number of objects
%%   in the image, and is the upper bound on performance of all possible
%%   algorithms.} 
%% \label{fig:sum_iu_instances}
%% \end{figure}
%Annotation across all class labels and all object instances is a tedious task. The scene parsing requires a dataset of nearly fully labeled images ($>75\%$ of pixels per image), and our object detector requires the labeling to \textbf{separate} each instance from others, which many datasets lack when objects of the same class occur adjacent to one another.  As it had full scene labeling already, 

%, as well as added to the label set: \texttt{person}, \texttt{vehicle}, \texttt{boat}, \texttt{ground}, an \texttt{vegetation}, fo  
We investigate the region generating methods of SCALPEL \cite{weiss2013scalpel} and Selective Search \cite{uijlings2013selective}, and in Figure~\ref{fig:lmsun_abo_and_lp} compare our chunk generating method against them on our LM+Sun Adjacent Cars dataset with the Average Best Object method suggested by \cite{weiss2013scalpel}, and additionally train our system by using these methods to fill the candidate pool. In Table~\ref{tab:sum_iu_sbd}, we compare different list predictions methods on \texttt{vehicle} and \texttt{person} data, respectively.



%% In the \vocperson\, experiment, we
%% trained two separate list predictors: one with the candidate pool
%% filled by the chunk grower, and one with the candidate pool filled by
%% the class-agnostic approach detailed in 
%% (Selective Search), and find that our list predictor built with grown
%% chunks outperforms all baselines, and the list predictor built with
%% selective search chunks outperforms two of the three baselines. %% In
%% Figure~\ref{fig:sum_iu_instances}, we test the performance of our
%% system in several different budget scenarios: 1) the predicted list
%% length, $k$, is greater than the number of instances in an image, $m$,
%% and 2) $k = m$. In these experiments, $k = 3$, and $m = \{1, 2,
%% 3\}$. At each value of $m$, we test on the subset of images containing
%% exactly $m$ instances. These experiments show that the list predictor
%% armed with our grown chunks outperforms the baseline approaches even
%% in sparsely populated instance settings.
%% In Figure~\ref{fig:pr_curve},
%% we plot the region-based Precision/Recall performance trade-off of our
%% methods versus the most competitive baseline for each. 
%% In Figure~\ref{fig:result_pic2}, we show additional qualitative results.








\begin{figure}[t]

        \centering
        \tabcolsep=0.02cm
        \setlength\extrarowheight{2pt}
        %% \vspace{20pt}
         \captionof{table}{List prediction and baseline performance on VOC2012 Person validation data and an 80/20 split of SBD Vehicles. Our list prediction outperforms all baselines in both experiments. In SBD Vehicles, the most competitive is the Scene Parsing intersected with DPM Bounding boxes. In VOC2012 Person, scene parsing was lower quality, and resulted in the DPM Boxes outperforming other baselines.} \label{tab:sum_iu_sbd}
         \begin{tabular}{|l||c|c|c|c|c||c|c|c|}
\cline{2-9}
\multicolumn{1}{c||}{} & \multicolumn{5}{c||}{SBD Vehicle} & \multicolumn{3}{c|}{VOC2012 Person} \\
\cline{2-9}
\multicolumn{1}{c||}{} & $f_{\text{L[0]}}$ & $f_{\text{L[0:1]}}$ & $f_{\text{L[0:2]}}$ & $f_{\text{L[0:3]}}$ & $f_{\text{L[0:4]}}$ &$f_{\text{L[0]}}$ & $f_{\text{L[0:1]}}$ & $f_{\text{L[0:2]}}$ \\
\hline
$\overline{R(c^*)}$ & 0.82 & 1.43 & 1.87 & 2.19 & 2.44 &  0.83 & 1.17 & 1.33 \\
\hline
$\overline{R(c_\mathcal{G}^*)}$  & 0.69 & 1.14 & 1.45 & 1.66 & 1.81 &  0.52 & 0.71 & 0.79 \\
\hline
\multicolumn{9}{c}{}\\[-10pt]
\hline
VC & \textbf{0.58} & \textbf{0.89} & \textbf{1.08} & \textbf{1.18} & \textbf{1.25}& \textbf{0.38} & \textbf{0.50} & \textbf{0.53} \\
\hline
VC w. SS & - & - & - & - & - &  0.27 & 0.36 & 0.41 \\
\hline
SP $\cap$ DPM  & 0.56 & 0.79 & 0.91 & 1.02 & 1.07  & 0.16 & 0.19 & 0.21 \\
\hline
CC & 0.37 & 0.53 & 0.60 & 0.65 & 0.66 & 0.19 & 0.24 & 0.27 \\
\hline
DPM & 0.28 & 0.39 & 0.43 & 0.45 & 0.47 &  0.29 & 0.38 & 0.41 \\
\hline
\end{tabular}
\end{figure}

    %% \subfloat[][\tiny LM+Sun Adjacent Cars performance of best candidate lists (solid lines) and predicted candidate lists. Our chunk generating method generates candidates of similar quality to that of SCALPEL. On this dataset, our baselines perform quite well, but the best performing list predictor is that which uses our baseline chunks as the candidate pool, and essentially reorders them. We also demonstrate that our learning method is compatible with other candidate pools, using both SCALPEL and Selective Search generating methods for building list predictors.]{
%%        \begin{minipage}[t]{
%%             \lmsunwidth}
%%             \centering
%% \vspace{0pt}
%%             %% \includegraphics[width=\textwidth]{img/lmsun_ac/with_legend_sum_iu_during_testing_with_conncomp.png}
%%             %% \includegraphics[width=\textwidth]{img/lmsun_ac/with_legend_sum_iu_during_testing_v8.png}
%%             \includegraphics[width=\textwidth]{img/lmsun_ac/with_legend_sum_iu_during_testing_v7.png}
%%     %% \caption{\tiny Performance of lists constructed from best candidates from each prediction pool (solid lines) and predicted candidates (dotted lines). Our chunk generating method (dark blue) generates candidates of similar quality to that of SCALPEL (light blue). On this dataset, our DPM-based baselines (magenta and dark cyan) perform quite well, but the best performing prediction method (dotted green line) is the list predictor that uses the SP $\cap$ DPM chunks as the candidate pool, and essentially has learned to reorders them. Additionally, we use Selective Search (red) as a candidate pool generating method.} \label{fig:sum_iu_lmsun}
%%     \caption{ $f(L; G)$ performance of lists constructed from best candidates from each prediction pool (dashed lines) and predicted candidates (solid lines) on a 50/50 split of LM+Sun Adjacent Cars dataset. Our chunk generating method (dark blue) generates candidates of similar quality to that of SCALPEL (light blue). On this dataset, our DPM-based baselines (magenta and dark cyan) perform quite well, but the best performing list prediction method (green line) is our list predictor that uses the SP $\cap$ DPM chunks as the candidate pool, and essentially has learned how to reorder them. This demonstrates how our approach can utilize and improve different candidate sources.} \label{fig:sum_iu_lmsun}
%%             \end{minipage} \\

%%% SBD vehicles
%% \subfloat[][\tiny SBD Vehicles performance. Our List Prediction outperforms all baselines, the most competitive of which is the Scene Parsing intersected with DPM Bounding boxes.]{
%%         \begin{minipage}[t]{
        %% \lmsunwidth}
        %% \centering
        %% \tabcolsep=0.02cm
        %% \setlength\extrarowheight{2pt}
%%         \captionof{table}{SBD Vehicles performance. Our List Prediction outperforms all baselines, the most competitive of which is the Scene Parsing intersected with DPM Bounding boxes} \label{tab:sum_iu_sbd}
%% \tiny
%%         \begin{tabular}{|c||c|c|c|c|c|}
%% \hline
%%  &$f_{\text{L[0]}}$ & $f_{\text{L[0:1]}}$ & $f_{\text{L[0:2]}}$ & $f_{\text{L[0:3]}}$ & $f_{\text{L[0:4]}}$ \\
%% \hline
%% $\overline{R(c^*)}$ (mean optimal) & 0.82 & 1.43 & 1.87 & 2.19 & 2.44 \\
%% \hline
%% $\overline{R(c_\mathcal{G}^*)}$ (mean best candidate) & 0.69 & 1.14 & 1.45 & 1.66 & 1.81 \\
%% \hline
%% \hline
%% List Prediction, Grown \& Baseline Chunks & \textbf{0.58} & \textbf{0.89} & \textbf{1.08} & \textbf{1.18} & \textbf{1.25} \\
%% \hline
%% SP $\cap$ DPM Baseline & 0.56 & 0.79 & 0.91 & 1.02 & 1.07 \\
%% \hline
%% Connected Components Baseline & 0.37 & 0.53 & 0.60 & 0.65 & 0.66 \\
%% \hline
%% DPM Boxes Baseline & 0.28 & 0.39 & 0.43 & 0.45 & 0.47 \\
%% \hline
%% \end{tabular}
%% \end{minipage}
%% \hfill
%%         \begin{minipage}[t]{
%%         \lmsunwidth}
%%         \centering
%%         \tabcolsep=0.06cm
%%         \setlength\extrarowheight{2pt}
%% \captionof{table}{VOC2012 Person evaluation. Scene parsing was not as high quality as it was in the other experiments, so baselines based on it suffered. List prediction outperformed all baselines.} \label{tab:sum_iu_voc}
%% \tiny        
%%         \begin{tabular}{|c||c|c|c|}
%% \hline
%%  & $f_{\text{L[0]}}$ & $f_{\text{L[0:1]}}$ & $f_{\text{L[0:2]}}$ \\
%% \hline
%% $\overline{R(c^*)}$ (mean optimal) & 0.83 & 1.17 & 1.33 \\
%% \hline
%% $\overline{R(c_\mathcal{G}^*)}$ (mean best candidate) & 0.52 & 0.71 & 0.79 &  & 0.52 & 0.71 & 0.79 \\
%% \hline
%% \hline
%% Predicted Grown Chunks & \textbf{0.38} & \textbf{0.50} & \textbf{0.53} \\
%% \hline
%% DPM Boxes Baseline & 0.29 & 0.38 & 0.41 \\
%% \hline
%% List Prediction with Selective Search & 0.27 & 0.36 & 0.41 \\
%% \hline
%% Connected Components Baseline & 0.19 & 0.24 & 0.27 \\
%% \hline
%% SP $\cap$ DPM Baseline & 0.16 & 0.19 & 0.21 \\
%% \hline
%% \end{tabular}
%% \end{minipage}





%% \begin{figure}[h!]
%%         %% \tiny
%%         \centering
%%     %% \subfloat[][\tiny LM+Sun Adjacent Cars candidate quality. A previously proposed metric for candidate pool quality is Average Best Overlap (ABO), in which the best overlapping candidate for every ground truth object is computed, and then averaged across the dataset. We find that our grown chunks generally outperform the Selective Search and SCALPEL methods ]{
%% \vspace{-20pt}
%%         \begin{minipage}[t]{
%%             \lmsunwidth}       
%%             \centering
%%             \includegraphics[width=\textwidth]{abo/abo_all_methods.png}
%%     %% \caption{\tiny LM+Sun Adjacent Cars candidate quality, measured by Average Best Overlap (ABO). We find that our grown chunks generally outperform the Selective Search and SCALPEL methods} \label{fig:lmsun_abo_and_lp}
%%     \caption{LM+Sun Adjacent Cars candidate quality, measured by Average Best Overlap (ABO). We find that our grown chunks generally outperform the Selective Search and SCALPEL methods} \label{fig:lmsun_abo_and_lp}

%%         \centering
%%         \tabcolsep=0.02cm
%%         \setlength\extrarowheight{2pt}
%%         \tiny
%%          \captionof{table}{SBD Vehicles performance. Our List Prediction outperforms all baselines, the most competitive of which is the Scene Parsing intersected with DPM Bounding boxes} \label{tab:sum_iu_sbd}
%%         \begin{tabular}{|c||c|c|c|c|c|}
%% \hline
%%  &$f_{\text{L[0]}}$ & $f_{\text{L[0:1]}}$ & $f_{\text{L[0:2]}}$ & $f_{\text{L[0:3]}}$ & $f_{\text{L[0:4]}}$ \\
%% \hline
%% $\overline{R(c^*)}$ (mean optimal) & 0.82 & 1.43 & 1.87 & 2.19 & 2.44 \\
%% \hline
%% $\overline{R(c_\mathcal{G}^*)}$ (mean best candidate) & 0.69 & 1.14 & 1.45 & 1.66 & 1.81 \\
%% \hline
%% \hline
%% List Prediction, Grown \& Baseline Chunks & \textbf{0.58} & \textbf{0.89} & \textbf{1.08} & \textbf{1.18} & \textbf{1.25} \\
%% \hline
%% SP $\cap$ DPM Baseline & 0.56 & 0.79 & 0.91 & 1.02 & 1.07 \\
%% \hline
%% Connected Components Baseline & 0.37 & 0.53 & 0.60 & 0.65 & 0.66 \\
%% \hline
%% DPM Boxes Baseline & 0.28 & 0.39 & 0.43 & 0.45 & 0.47 \\
%% \hline
%% \end{tabular}
%%         \end{minipage}
%%        \quad
%%     %% \subfloat[][\tiny LM+Sun Adjacent Cars performance of best candidate lists (solid lines) and predicted candidate lists. Our chunk generating method generates candidates of similar quality to that of SCALPEL. On this dataset, our baselines perform quite well, but the best performing list predictor is that which uses our baseline chunks as the candidate pool, and essentially reorders them. We also demonstrate that our learning method is compatible with other candidate pools, using both SCALPEL and Selective Search generating methods for building list predictors.]{
%%        \begin{minipage}[t]{
%%             \lmsunwidth}
%%             \centering
%%             \includegraphics[width=\textwidth]{img/lmsun_ac/with_legend_sum_iu_during_testing_with_conncomp.png}
%%     %% \caption{\tiny Performance of lists constructed from best candidates from each prediction pool (solid lines) and predicted candidates (dotted lines). Our chunk generating method (dark blue) generates candidates of similar quality to that of SCALPEL (light blue). On this dataset, our DPM-based baselines (magenta and dark cyan) perform quite well, but the best performing prediction method (dotted green line) is the list predictor that uses the SP $\cap$ DPM chunks as the candidate pool, and essentially has learned to reorders them. Additionally, we use Selective Search (red) as a candidate pool generating method.} \label{fig:sum_iu_lmsun}
%%     \caption{Performance of lists constructed from best candidates from each prediction pool (solid lines) and predicted candidates (dotted lines). Our chunk generating method (dark blue) generates candidates of similar quality to that of SCALPEL (light blue). On this dataset, our DPM-based baselines (magenta and dark cyan) perform quite well, but the best performing prediction method (dotted green line) is the list predictor that uses the SP $\cap$ DPM chunks as the candidate pool, and essentially has learned to reorders them. Additionally, we use Selective Search (red) as a candidate pool generating method.} \label{fig:sum_iu_lmsun}
%%             \end{minipage} \\

%% %%% SBD vehicles
%% %% \subfloat[][\tiny SBD Vehicles performance. Our List Prediction outperforms all baselines, the most competitive of which is the Scene Parsing intersected with DPM Bounding boxes.]{
%% %%         \begin{minipage}[t]{
%%         %% \lmsunwidth}
%%         %% \centering
%%         %% \tabcolsep=0.02cm
%%         %% \setlength\extrarowheight{2pt}
%% %%         \captionof{table}{SBD Vehicles performance. Our List Prediction outperforms all baselines, the most competitive of which is the Scene Parsing intersected with DPM Bounding boxes} \label{tab:sum_iu_sbd}
%% %% \tiny
%% %%         \begin{tabular}{|c||c|c|c|c|c|}
%% %% \hline
%% %%  &$f_{\text{L[0]}}$ & $f_{\text{L[0:1]}}$ & $f_{\text{L[0:2]}}$ & $f_{\text{L[0:3]}}$ & $f_{\text{L[0:4]}}$ \\
%% %% \hline
%% %% $\overline{R(c^*)}$ (mean optimal) & 0.82 & 1.43 & 1.87 & 2.19 & 2.44 \\
%% %% \hline
%% %% $\overline{R(c_\mathcal{G}^*)}$ (mean best candidate) & 0.69 & 1.14 & 1.45 & 1.66 & 1.81 \\
%% %% \hline
%% %% \hline
%% %% List Prediction, Grown \& Baseline Chunks & \textbf{0.58} & \textbf{0.89} & \textbf{1.08} & \textbf{1.18} & \textbf{1.25} \\
%% %% \hline
%% %% SP $\cap$ DPM Baseline & 0.56 & 0.79 & 0.91 & 1.02 & 1.07 \\
%% %% \hline
%% %% Connected Components Baseline & 0.37 & 0.53 & 0.60 & 0.65 & 0.66 \\
%% %% \hline
%% %% DPM Boxes Baseline & 0.28 & 0.39 & 0.43 & 0.45 & 0.47 \\
%% %% \hline
%% %% \end{tabular}
%% %% \end{minipage}
%% \hfill
%%         \begin{minipage}[t]{
%%         \lmsunwidth}
%%         \centering
%%         \tabcolsep=0.06cm
%%         \setlength\extrarowheight{2pt}
%% \captionof{table}{VOC2012 Person evaluation. Scene parsing was not as high quality as it was in the other experiments, so baselines based on it suffered. List prediction outperformed all baselines.} \label{tab:sum_iu_voc}
%% \tiny        
%%         \begin{tabular}{|c||c|c|c|}
%% \hline
%%  & $f_{\text{L[0]}}$ & $f_{\text{L[0:1]}}$ & $f_{\text{L[0:2]}}$ \\
%% \hline
%% $\overline{R(c^*)}$ (mean optimal) & 0.83 & 1.17 & 1.33 \\
%% \hline
%% $\overline{R(c_\mathcal{G}^*)}$ (mean best candidate) & 0.52 & 0.71 & 0.79 \\
%% \hline
%% \hline
%% List Prediction, Grown \& Baseline Chunks & \textbf{0.38} & \textbf{0.50} & \textbf{0.53} \\
%% \hline
%% DPM Boxes Baseline & 0.29 & 0.38 & 0.41 \\
%% \hline
%% List Prediction with Selective Search & 0.27 & 0.36 & 0.41 \\
%% \hline
%% Connected Components Baseline & 0.19 & 0.24 & 0.27 \\
%% \hline
%% SP $\cap$ DPM Baseline & 0.16 & 0.19 & 0.21 \\
%% \hline
%% \end{tabular}


%% \end{minipage}

%% \end{figure}


%%%% images

%% \begin{table}[h!]
%% \begin{center}
%% \tabcolsep=0.05cm
%% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%% \multirow{2}{*}[\doubleoffset]{\includegraphics[width=\vocsinglewidth]{img/voc_single/bottle_1overlay.png}} & \multirow{2}{*}[\doubleoffset]{\includegraphics[width=\vocsinglewidth]{img/voc_single/pottedplant_1overlay.png}} \includegraphics[width=\vocsinglewidth]{img/voc_single/aeroplane_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/bird_1overlay.png}  &   \multicolumn{2}{b{1em}}{\includegraphics[width=1.5\vocsinglewidth]{img/voc_single/bus_1overlay.png}}  &\hspace{-4em}   \includegraphics[width=\vocsinglewidth]{img/voc_single/chair_1overlay.png}  &   \includegraphics[width=\vocsinglewidth]{img/voc_single/dog_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/motorbike_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/sheep_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/table_1overlay.png}\\
%% \hline
%%  & \hspace{4em} \includegraphics[width=\vocsinglewidth]{img/voc_single/bicycle_1overlay.png} &  \includegraphics[width=\vocsinglewidth]{img/voc_single/boat_1overlay.png} & \includegraphics[width=\vocsinglewidth]{img/voc_single/cat_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/cow_1overlay.png}&   \includegraphics[width=\vocsinglewidth]{img/voc_single/horse_1overlay.png}&   \includegraphics[width=\vocsinglewidth]{img/voc_single/person_1overlay.png}&   \includegraphics[width=\vocsinglewidth]{img/voc_single/sofa_1overlay.png}&   \includegraphics[width=\vocsinglewidth]{img/voc_single/train_1overlay.png}\\
%% \end{tabular}
%% \end{center}
%% \end{table}


\newlength{\vocsinglewidth}
\setlength{\vocsinglewidth}{.10\textwidth}
\newlength{\doubleoffset}
\setlength{\doubleoffset}{2\normalbaselineskip}

%% \vspace{-25pt}
\begin{figure}[h!]
\tabcolsep=0.07cm
\centering
\begin{tabular}{cccccccc}
\multirow{2}{*}[\doubleoffset]{\includegraphics[width=\vocsinglewidth]{img/voc_single/bottle_1overlay.png}}  & \includegraphics[width=\vocsinglewidth]{img/voc_single/chair_1overlay.png}  &   \includegraphics[width=\vocsinglewidth]{img/voc_single/sheep_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/bird_1overlay.png} & \includegraphics[width=\vocsinglewidth]{img/voc_single/cat_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/cow_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/tvmonitor_1overlay.png} & \multirow{2}{*}[\doubleoffset]{\includegraphics[width=\vocsinglewidth]{img/voc_single/pottedplant_1overlay.png}}\\   
 & \includegraphics[width=\vocsinglewidth]{img/voc_single/table_1overlay.png} & \includegraphics[width=\vocsinglewidth]{img/voc_single/dog_1overlay.png} & \includegraphics[width=\vocsinglewidth]{img/voc_single/train_1overlay.png} &   \includegraphics[width=\vocsinglewidth]{img/voc_single/motorbike_1overlay.png} & \includegraphics[width=\vocsinglewidth]{img/voc_single/person_1overlay.png}   &  \includegraphics[width=\vocsinglewidth]{img/voc_single/sofa_1overlay.png} \\
 \includegraphics[width=\vocsinglewidth]{img/voc_single/car_1overlay.png} &    \includegraphics[width=\vocsinglewidth]{img/voc_single/bicycle_1overlay.png}&   \includegraphics[width=\vocsinglewidth]{img/voc_single/horse_1overlay.png} & \multirow{1}{*}[1.23\doubleoffset]{\includegraphics[width=\vocsinglewidth]{img/voc_single/aeroplane_1overlay.png}} &  \multirow{1}{*}[1.23\doubleoffset]{\includegraphics[width=\vocsinglewidth]{img/voc_single/boat_1overlay.png}}   &   \multicolumn{2}{p{1em}}{\multirow{1}{*}[1.23\doubleoffset]{\includegraphics[width=1.5\vocsinglewidth]{img/voc_single/bus_1overlay.png}}} \\% 
\end{tabular}\captionof{figure}{Example single predictions on PASCAL VOC2012}\label{fig:voc2012}

\tabcolsep=0.09cm
\captionof{table}{Average instance-based accuracy (a metric proposed by \cite{yang2012layered}), and first slot scores (corresponding to the average overlap of the first prediction in each image) for systems trained and tested on the standard PASCAL 2012 \texttt{train} and \texttt{val} sets. We find that the very small amount of co-occurring instance training data was not sufficient to enable our system to perform as well as it did in our other experiments on images with co-occurring instances. While \cite{yang2012layered} provides experimental results of average instance-based accuracy on PASCAL 2010, their results are confined to verified correct DPM detections, rendering a fair comparison difficult.} \label{tab:voc2012}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 & aeroplane & bicycle & bird & boat & bottle & bus  & car & cat & chair & cow \\
\hline
$\text{\text{inst}}_{\text{acc}}$ &.157 &.066    &.105 &.132 &   .079 &.228 &.097 & .155 & .071 & .211 \\
\hline
$f(L[0])$ &.521 &.148   &.375 &.335 & .186  &.439 &.190 &.445 &.141 & .494 \\
\hline
$f(L)$&  .530    &   .158  & .394 & .347 &.202&.509 & .195 & .461 & .171 & .581 \\
\hline
\end{tabular}
\vspace*{-5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\multicolumn{11}{l}{}\\[-5pt]
\hline
 & diningtable & dog  & horse & motorbike & person & pottedplant & sheep & sofa & train & tvmonitor \\
\hline
$\text{\text{inst}}_{\text{acc}}$ & .098       &.165 & .197 &.166      & .193  &    .078   & .182  &  .139 & .170  & .109  \\
\hline
$f(L[0])$  & .260       &.430 & .437 & .407     & .362    &  .133   & .466  & .260 & .403 & .270 \\
\hline
$f(L)$  & .261 & .454      & .479 &  .441    & .456   &  .160    & .582 &  .272    & .409 & .278 \\
\hline
%% \multicolumn{11}{l}{\tiny \textsuperscript{*} Predictions made with model trained on LM+Sun Adjacent Cars dataset}
\end{tabular}
\vfill
\normalsize
\end{figure}

%% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%% \hline
%%                           & aeroplane & bicycle & bird & boat & bottle & bus  & car & car\textsuperscript{*} & cat & chair & cow & diningtable & dog  & horse & motorbike & person & pottedplant & sheep & sofa & train & tvmonitor\\
%% \hline
%% $\text{\text{inst}}_{\text{acc}}$ &.157 &.066    &.105 &.132 &   .079 &.228 &.097 & .117  &.155 &.071 & .211& .098       &.165 & .197 &.166      & .193  &    .078   & .182  &  .139 & .170  & .109  \\
%% \hline
%% $f(L[0]\text{;} G)$ &.502 &.137   &.336 &.317 &  .151  &.419 &.170 &.200 &.396        &.104 & .461& .243       &.401 & .416 &                  .387     & .382    &  .107   & .413  & .233 & .390 & .242 \\
%% \hline
%% $f(L\text{;} G)$           &  .653    &   .192  & .484 & .422 &  .242  & .614 & .241 & .316 & .566 & .196 & .704  & .325 & .553      & .586 &  .542      & .533   &  .183    & .679 &  .334    & .508 & .340 \\
%% \hline
%% \multicolumn{21}{l}{\tiny \textsuperscript{*} Predictions made with model trained on LM+Sun Adjacent Cars dataset}\\

%% \end{tabular}


%% \begin{table}
%% \tiny
%% \tabcolsep=0.05cm
%% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%%                         & aeroplane & bicycle & bird & boat & bottle & bus  & car  & cat & chair & cow & diningtable & dog  & horse & motorbike & person & pottedplant & sheep & sofa & train & tvmonitor\\
%% \hline
%% $\text{\text{inst}}_{\text{acc}}$     & 0.249 & 0.070   & 0.120 & 0.205 & 0.090   & 0.335 & 0.134 & 0.220 & 0.087 & 0.268 & 0.105       & 0.157 &      & 0.186        &        & 0.091       &    0.160 & 0.086 &     & 0.157 \\
%% \hline
%% $\text{\text{inst}}_{\text{best}}$ & 0.510& 0.207   & 0.308 &  0.424 & 0.168   & 0.543 & 0.353 & 0.471 & 0.170 & 0.484 & 0.382       & 0.437 &     & 0.431         & 0.242   & 0.447       & 0.325    & 0.323  &    & 0.359 \\
%% \end{tabular}
%% \normalsize
%% \end{table}

%% \newlength{\combosumiulength}
%% \setlength{\combosumiulength}{.45\textwidth}
%% \newlength{\legendlength}
%% \setlength{\legendlength}{.3\textwidth}
%% \begin{figure}[h!]
%%         \tiny
%%         \centering

%%         \subfloat[][SBD \texttt{vehicle} performance]{\includegraphics[width=\combosumiulength]{img/fixed_vehicle/sum_iu_during_test_fold_2_5_rounds_overlayed.png} \label{subfig:sum_iu_all_sbd_vehicle}}
%%         \subfloat[][VOC 2012 \texttt{person} performance]{\includegraphics[width=\combosumiulength]{img/fixed_voc_person/sum_iu_During_Testing_with_ss_overlayed.png} \label{subfig:sum_iu_all_voc_person}} \\
%%          %% \subfloat[][Legend]{\includegraphics[width=\legendlength]{img/sum_iu_legend_with_ss_cropped.png} \label{subfig:sum_iu_legend_all}}

%%         %% \subfloat[][Performance on 1-instance images]{\includegraphics[width=.30\textwidth]{img/sum_iu_During_Testing_3-3-19-33_1prediction_budget_SBD_VEHICLE_FOLD2.png}} \qquad
%%         %% \subfloat[][Performance on 2-instance images]{\includegraphics[width=.30\textwidth]{img/sum_iu_During_Testing_3-3-19-33_2prediction_budget_SBD_VEHICLE_FOLD2.png}} \qquad
%%         %% \subfloat[][Performance on 3-instance images]{\includegraphics[width=.30\textwidth]{img/sum_iu_During_Testing_3-3-19-33_3prediction_budget_SBD_VEHICLE_FOLD2.png}}
%% \caption{\emph{Sum \iou of List} vs. \emph{Length of prediction list}
%%   of different detection list building methods on  SBD
%%   \texttt{vehicle} and PASCAL VOC 2012 \texttt{person} images. As detections are appended to each list, the resulting score (the
%%   y-axis; the evaluation of Equation \ref{list_obj_func}) of the list
%%   grows. The list built with the optimal combinations of superpixels is an upper bound given
%%   segmentation. The list built with the best grown
%%   chunks demonstrates that our
%%   method for growing adds high-quality chunks to the candidate
%%   set. Our list predictor outperforms the three baselines. %(magenta, cyan, and black dotted lines). 
%% In the ideal case, the list predictor would choose
%%   the best chunks from the candidate pool, and the predicted chunks
%%   line would exactly match the best grown chunks line. For the SBD
%%   \texttt{vehicle} test (Figure \ref{subfig:sum_iu_all_sbd_vehicle}),
%%   we find that both the connected components of scene parsing and the
%%   DPM bounding boxes perform adequately, which yields good performance
%%   for our most sophisticated baseline: scene parsing intersected with
%%   connected components. For the PASCAL VOC \texttt{person} test (Figure
%%   \ref{subfig:sum_iu_all_voc_person}), we find that the scene parsing
%%   is relatively lackluster, which degrades the performance of the
%%   intersection baseline. Importantly, we also observe reasonable
%%   performance in the case of building a list predictor from
%%   class-agnostic chunks from selective search\cite{uijlings2013selective},
%%   demonstrating that our generic framework can use input from methods
%%   besides our own. } \label{fig:sum_iu_all}
%% \end{figure}

%% \subsection{Features for List Predictor} \label{sec:features}
\subsection{Features}\label{sec:features}
As discussed in \ref{sec:list_learning}, the features $\Phi(c,L)$ should encode the \emph{quality} of a chunk $c$ (e.g. ``Does the chunk look like a vehicle?'') and \emph{similarity} with the currently predicted list $L$ (e.g. ``Is this chunk similar to previously predicted chunks'' ). 
One of the quality features is built upon the superpixel-wise
multi-class label distribution from \cite{munoz-eccv-10}, where we
compute label distribution for each chunk via aggregating histograms
of its constituent superpixels. The other quality features are shape
features including central moments of the chunk, area, and scale
relative to the image. The similarity features we use primarily encode
spatial information between predictions. We use a candidate's
$\frac{I}{U}$ with previous predictions, the spatial histogram used in
\cite{desai2011discriminative} and the size of the current list. Chunks with high similarity
with previously predicted chunks in the list are less favored.

%% \begin{figure}[h!]
%% \centering
%% %% \includegraphics[width=.3\textwidth]{img/old_supplementary/6000249_1overlayed.png} \includegraphics[width=.3\textwidth]{img/old_supplementary/6000249_2overlayed.png} 
%% \includegraphics[width=.3\textwidth]{img/old_supplementary/6000249_3overlayed.png}
%% \includegraphics[width=.3\textwidth]{img/old_supplementary/6000199_5overlayed.png}
%% \includegraphics[width=.3\textwidth]{img/6000186_3overlayed.png}
%%  \includegraphics[width=.3\textwidth]{img/extra_qualitative_results/2007_007649_2overlay_pred.png}
%%  \includegraphics[width=.3\textwidth]{img/extra_qualitative_results/2008_000588_2overlay_pred.png}
%%  \includegraphics[width=.3\textwidth]{img/extra_qualitative_results/2008_002864_2overlay_pred.png}\\
%%  \includegraphics[width=.3\textwidth]{img/extra_qualitative_results/2007_003191_1overlay_pred.png}
%% \includegraphics[width=.3\textwidth]{img/6000343_1overlayed.png}
%% \includegraphics[width=.3\textwidth]{img/old_supplementary/6000147_3overlayed.png}
%% %% \includegraphics[width=.3\textwidth]{img/old_supplementary/6000340_1overlayed.png} \includegraphics[width=.3\textwidth]{img/old_supplementary/6000340_2overlayed.png} 
%% %% \includegraphics[width=.3\textwidth]{img/old_supplementary/6000340_3overlayed.png}\\
%% %% \includegraphics[width=.19\textwidth]{img/old_supplementary/6000199_1overlayed.png} \includegraphics[width=.19\textwidth]{img/old_supplementary/6000199_2overlayed.png} \includegraphics[width=.19\textwidth]{img/old_supplementary/6000199_3overlayed.png} \includegraphics[width=.19\textwidth]{img/old_supplementary/6000199_4overlayed.png}


%% \hfill
%% \caption{Additional qualitative results of running our list prediction and candidate generation methods on test data. }
%% \label{fig:result_pic2}
%% \end{figure}

%% \subsection{Features for Grower} \label{sec:feature_grower}
The features $\theta(s,c')$ for the grower encode information about the quality of proposed chunk $c' = c \cup \{s\}$ by growing $c$ with superpixel $s$. The grower uses the same quality features that characterize $c'$ used by the list predictor, as well as several of the class-agnostic features described in \cite{uijlings2013selective}, specifically color similarity (color histogram intersection), which encourages regions to be built from similarly colored regions, and region fill, which encourages growing compact chunks. See \cite{uijlings2013selective} for further details. As each superpixel is iteratively added to the chunk, similarity to the growing chunk for remaining candidate superpixels is recomputed. %% In the case of person detection, we utilized a face detector and built a feature to track the current face detection memberships of the growing chunks. During training, if a growing chunk currently overlaps a face detection, candidate superpixels within a separate face detection will have target scores of 0, as they correspond to a separate person instance. %%%not used for current results
\input{us_vs_them_all}
%% \begin{figure}[h!]
%% \caption{Sum of I/U v.s. Length of prediction list on 712 training, 176 testing images (80\% train, 20\% test) on PASCAL VOC \texttt{person}. } \label{fig:sum_iu}
%% \end{figure}
%% \begin{figure}[h!]
%%         \centering
%% % \subfloat[][PR with Baseline Region I/U]{\includegraphics[width=.5\textwidth]{img/fixed_vehicle/PR_3_predictions_3orless_3-6-17-36.png} \label{subfig:sbd_vehicle_pr}}
%% % \subfloat[][PR with Baseline Region I/U]{\includegraphics[width=.5\textwidth]{img/fixed_voc_person/with_legend_PR_3_predictions_3orless_3-6-17-32.png} \label{subfig:voc_person_pr}}
%%  \subfloat[][PR curve comparison on SBD vehicle class ]{\includegraphics[width=.4\textwidth]{img/fixed_vehicle/PR_3_predictions_3-6-17-48_lenient_recall.png} \label{subfig:sbd_vehicle_pr}}
%%  \subfloat[][PR curve comparison on VOC 2012 person class]{\includegraphics[width=.4\textwidth]{img/fixed_voc_person/PR_3_predictions_3-6-17-52_lenient_recall.png} \label{subfig:voc_person_pr}}
%%  %%\subfloat[][PR with Baseline Box I/U]{\includegraphics[width=.5\textwidth]{img/vocperson_pr/PR_3_predictions_bbox_iu_3-5-19-23.png}} \\
%%  %%\subfloat[][PR with Baseline Box I/U]{\includegraphics[width=.5\textwidth]{img/sbdvehicle_pr/PR_3_predictions_bbox_GT_3-5-20-1.png}}
%% %\end{subfigure}
%% \caption{Precision-Recall curves of models corresponding to SBD
%%   \texttt{vehicle} test (Figure~\ref{subfig:sbd_vehicle_pr}), and
%%   PASCAL VOC 2012 \texttt{person} test
%%   (Figure~\ref{subfig:voc_person_pr}). For each test, we compare with
%%   our most competitive baseline (scene parsing intersected with DPM
%%   for \texttt{vehicle}, and DPM for \texttt{person}). Each plot
%%   displays three different true positive thresholds for the dueling
%%   methods: $0.3, 0.4, 0.5$ I/U. The baseline methods are displayed as
%%   dotted curves, and our list prediction method is displayed as a
%%   solid curve. Because lists are of size-3, if an image has more than three instances, we do not count additional unpredicted instances as false negatives
%% } \label{fig:pr_curve}%Our method outperforms the best baseline (scene parsing intersected with DPM) at all levels of I/U threshold.}
%% \end{figure}
%In Figure \ref{fig:num_pixels_vs_iu}, we see that it is difficult for all methods to cover ground truth instances when they are small. This is to be expected, as any undersegmentation results in an inability to cover the ground truth well. When the instances are larger, we see that the best generated chunks perform quite well, and the predicted chunks perform reasonably well.
%% In Figure~\ref{fig:us_vs_them_all}, we visually compare our predicted list of size three (solid lines) with the baseline models (dotted lines). The examples we give are objects with close proximity and it can be seen that our model performs better in reasoning about multiple objects. In Figure \ref{fig:sum_iu_all}, we show the sum of I/U score of the list as a function of list length. Note that some of the images contain only one instance. Figure \ref{fig:pr_curve} shows the precision-recall curve with different threshold and size of the list, which again demonstrates the accuracy of our model. 
 %% The red line shows the optimal chunk that can be possibly grown from the superpixels given access to the ground truth, which can be treated as an upper bound performance of any algorithm that is based on this fixed superpixel segmentation. The green line shows the optimal chunk among the grown candidate set chunk given access to the ground truth. Our grower therefore performs quite well, almost always generating candidates that overlap highly with the ground truth. All the other lines correspond to applying different models at test time without access to ground truth instances. Our model based on applying list predictor on the growned chunks, as illustrated in the blue line,  outperforms all baselines by a significant margin including the sophisticated model that uses intersection of DPM with HIM.
%\begin{figure}[h!] 
%\begin{subfigure}[h!]{0.8\textwidth}
%\centering
%\includegraphics[width=.8\textwidth]{img/num_pixels_small_vs_iu.png} 
%\caption{Performance on small objects. For very small objects, the segmentation is not fine enough, and results in object clipping. Any ground truth inexactness further compounds the difficulty of scoring high on small objects.}
%\end{subfigure}
%\centering
%\begin{subfigure}[h!]{0.8\textwidth}
%\centering
%\includegraphics[width=.8\textwidth]{img/num_pixels_vs_iu.png}
%\caption{Performance on all object sizes. For objects that aren't small, all types of chunks score reasonably high.}
%\end{subfigure}
%\caption{Ground truth instance sizes vs. optimal, optimal grown, and predicted chunks} \label{fig:num_pixels_vs_iu}
%\end{figure}


==> old_thesis_outline_flat.tex <==
\section{Introduction}
Many problem domains require learning and inference over combinatorial space.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 In extractive document summarization, we aim to choose the best subset of sentences to represent the article.  
\section{Related Work}
\section{Background}
\subsection{The Monotone Submodular List Function}
Let $\mathcal{S}$ denote the set of possible items to choose from
(\textbf{e.g.} ads, sentences, grasps) and $f$ be the utility list function that takes input of list $L \subseteq S$. Let $b(s|L) = f(L \oplus s) - f(L)$ denote the marginal benefit of adding the item $s$ to list $L$. %Our objective is to pick a list of
%items $L \subseteq \mathcal{S}$ to maximize a reward function $f$ that obeys the following properties:
We define monotonicty and submodularity of $f$ as follows: 
``Lists'' generalize the notion of ``set'' more commonly used in submodular optimization, and enables reasoning about item order and repeated items \cite{streeter2007online}. One may consider sets where appropriate.
  % We use ``list'' to convey an implicit notion of ordering (e.g., the order under which our model greedily chooses the list), but the reward function $f$ is computed over unordered sets.


\begin{enumerate}
\item \textbf{Monotonicity:} For any lists $L_1, L_2$, $f(L_1) \leq f(L_1 \oplus L_2)$ and $f(L_2) \leq f(L_1 \oplus L_2)$
\item \textbf{Submodularity:} For any lists $L_1,L_2$ and item $s \in \mathcal{S}$, $b(s|L_1) \geq b(s|L_1 \oplus L_2)$.
%, $f(L_1 \oplus s) - f(L_1) \geq f(L_1 \oplus L_2 \oplus s) - f(L_1 \oplus L_2)$. 
\end{enumerate}

Here, $\oplus$ denotes the concatenation operator. Intuitively, monotonicity
implies that adding more elements never hurts, and
submodularity captures the notion of diminishing returns (\emph{i.e.} adding an item
to a long list increases the objective less than when adding it to a shorter sublist). 
We further assume for simplicity that $f$ takes values in 
$[0,1]$, and that $f(\emptyset) = 0$ where $\emptyset$ denotes the empty
list. 

\subsection{Near-optimal Greedy Oracle Policy}
\[
\begin{aligned}
\text{maximize}_{L \subseteq V} && f(L)\\
\text{subject to } && L \in I\\
\end{aligned}
\]
, where $I$ is the set of all feasible sets subject to constraints. In this paper, we focus on the following three different constraints:
\begin{enumerate}
\item Cardinality constraint: Given some $k$, we have $ I = \{ S| S\subseteq V , |S| \leq k \}$.  \label{c}
\item Intersection of matroid constraints: Given $P$ matroid systems $(V, I_p)$, we have $I = \bigcap\limits_{p=1}^P I_p$. It can be seen that the cardinality constraint is a special case of single matroid constraint.
\item Knapsack constraint: Suppose each element $v\in V$ has non-uniform cost $\ell(v)$, let $\ell(S) = \sum_{i=1}^{|S|} \ell(s_i)$ denote the sum of cost of every element in $S$. Given a budget $B$, we have $I = \{S | S\subseteq V, \ell(S) \leq B \}$.
\end{enumerate}
For cardinality and intersection of matroid constraints, the greedy oracle policy starts with $L^G = \emptyset$ and sets
\begin{align}
 L^G = L^G \cup \{ \argmax\limits_{e\notin L^G: L^G\cup\{e\}\in I} b(e|L^G) \} 
\end{align}
until there does not exist an element $e$ that can be added to $L^G$ to create a feasible solution. It can be shown that for cardinality constrained problems:
$f(L^G) \geq (1-1/e) OPT$ \cite{nemhauser1978analysis}; and for problems subject to intersection of matroid constraints: $f(L^G) \geq \frac{1}{P+1} OPT$ \cite{fisher1978analysis}.

For knapsack constraint, we can simply replace marginal benefit by normalized marginal benefit (benefit cost ratio) to take cost into account. The cost-benefit greedy oracle policy starts with $L^G = \emptyset$ and iteratively adds element $e$ that maximize the normalized benefit among all elements that still fit into budget. 
\begin{align}
 L^G = L^G \cup \{ \argmax\limits_{e\notin L^G: L^G\cup\{e\}\in I} \frac{b(e|L^G)}{\ell(e)} \} 
\end{align}                                                     
%Define the marginal gain of adding element $e$ to a set $S$ as $\Delta(e|S) = f()$
%\subsection{The Context-Free Problem}
%\[
%\begin{aligned}
%\text{maximize}\qquad && f(S)\\
%\text{subject to }\qquad && w=b-s+w^0\\
%%\phantom{\text{subject to }} & l^b &\le b &\le u^b\\
%%\phantom{\text{subject to }} & l^s &\le s &\le u^s\\
%%\phantom{\text{subject to }} & l^{\text{bukd}} &\phantom{\le}  t(b+s) &\le u^t\\
%%\phantom{\text{subject to }} & l^{\text{bukd}} &\le A^{\text{dur}} w \text{ diag}(x^{\text{buk}}) &\le u^{\text{bukd}}\\
%%\phantom{\text{subject to }} & l^{\text{curp}} &\le A^{\text{dur}} w \text{ diag}(x^{\text{cur}}) &\le u^{\text{curp}}\\
%\end{aligned}
%\]

\subsection{Sampling and Near-optimality}
\begin{lemma} \label{lemAddList}
Let $\mathcal{S}$ be a feasible set and $f$ be a monotone submodular function defined on list of items from $\mathcal{S}$. For any lists $A,B$, we have that:
\begin{displaymath}
f(A \oplus B) - f(A) \leq |B| ( \mathbb{E}_{s \sim U(B)}[f(A \oplus s)] - f(A) )
\end{displaymath}
for $U(B)$ the uniform distribution on items in $B$. 
\end{lemma}
Note that any list sampled from $S$   Refer to \cite{ross2013learning} for proof. 
\begin{lemma} \label{lemStochasticRatio}
Let $\mathcal{S}$ be a set, and $f$ a monotone submodular function defined on lists of items in $\mathcal{S}$. Let $B$ be any list of items from $\mathcal{S}$ and $U(B)$ the uniform distribution on elements in $B$. Suppose we construct the list $A$ by sampling $k$ items randomly from $U(B)$ (with replacement). Denote $A_j$ the list obtained after $j$ samples, and $P_j$ the distribution over lists obtained after $j$ samples. Then:
\begin{displaymath}
\mathbb{E}_{A \sim P_k}[f(A)] \geq (1-(1-1/|B|)^k) f(B)
\end{displaymath}
In particular, for $k = |B|$:
\begin{displaymath}
\mathbb{E}_{A \sim P_k}[f(A)] \geq (1-1/e) f(B)
\end{displaymath}
\end{lemma}
%\begin{proof}
% By the monotone property and lemma \ref{lemAddList}, we have that for any list $A$: $f(B)-f(A) \leq f(A \oplus B) - f(A) \leq  |B| ( \mathbb{E}_{b \sim U(B)}[f(A \oplus b)] - f(A) )$. Because this holds for all lists, we must also have that for any distribution $P$ over lists $A$, $f(B) - \mathbb{E}_{A \sim P}[f(A)] \leq |B| \mathbb{E}_{A \sim P}[\mathbb{E}_{b \sim U(B)}[f(A \oplus b)] - f(A)]$. Also note that by the way we construct sets, we have that $\mathbb{E}_{A_{j+1} \sim P_{j+1}}[f(A_{j+1})] = \mathbb{E}_{A_j \sim P_j}[\mathbb{E}_{s \sim U(B)} [f(A_j \oplus s)]]$
%
%Now let $\Delta_j = f(B) - \mathbb{E}_{A_j \sim P_j}[f(A_j)]$. By the above we have that:
%\begin{displaymath}
%\begin{array}{rl}
%\multicolumn{2}{l}{\Delta_j}\\ 
%\leq & |B| \mathbb{E}_{A_j \sim P_j}[\mathbb{E}_{s \sim U(B)} [f(A_j \oplus s)] - f(A_j)] \\
%= & |B| \mathbb{E}_{A_j \sim P_j}[\mathbb{E}_{s \sim U(B)} [f(A_j \oplus s)]  - f(B) \\
%& + f(B) - f(A_j)] \\
%= & |B|( \mathbb{E}_{A_{j+1} \sim P_{j+1}}[f(A_{j+1)}]  - f(B) \\
%& + f(B) - \mathbb{E}_{A_j \sim P_j}[f(A_j)] )\\
%= &  |B| [\Delta_j - \Delta_{j+1} ] \\
%\end{array}
%\end{displaymath}
%Rearranging terms, this implies that $\Delta_{j+1} \leq (1-1/|B|) \Delta_j$. Recursively expanding this recurrence from $\Delta_k$, we obtain:
%\begin{displaymath}
%\Delta_{k} \leq (1-1/|B|)^k \Delta_0
%\end{displaymath}
%Using the definition of $\Delta_k$ and rearranging terms we obtain $E_{A \sim P_k}[f(A)] \geq (1-(1-1/|B|)^k) f(B)$. The second statement follows again from the fact that $(1-(1-1/|B|)^k) f(B) \geq (1-\alpha) f(B)$
%\end{proof}

\begin{corollary}
There exists a distribution that when sampled $k$ times to construct a list, achieves an approximation ratio of $(1-1/e)$ of the optimal list of size $k$ in expectation. In particular, if $A^*$ is an optimal list of size $k$, sampling $k$ times from $U(A^*)$ achieves this approximation ratio. Additionally, for any $\alpha \in (0,1]$, sampling $\lceil k\log(1/\alpha) \rceil$ times must construct a list that achieves an approximation ratio of $(1-\alpha)$ in expectation.
\end{corollary}
\begin{proof}
%Follows from the last lemma using $B=A^*$.
Refer to \cite{ross2013learning} for proof. 
\end{proof}

%This surprising result can also be seen as a special case of a more general result proven in prior related work that analyzed randomized set selection strategies to optimize submodular functions (lemma 2.2 in \cite{feige2011}). 

\subsection{The Contextual Learning Problem}
%\subsection{The Online Learning Problem}

We consider reward functions that may depend on some underlying state $x \in \mathcal{X}$ (e.g. a user, environment of the robot, a document, etc.). %, which is represented by a \emph{context}. 
Let $f_x$ denote the reward function for state $x$, and assume that $f_x$ is submodular. Our tasks is to construct good feasible list under some unknown distribution of states $D$ (e.g. distribution of users or documents we have to summarize). 
%monotone submodular for all $x$. Our task consists in learning to construct good lists of pre-specified length $k$ under some unknown distribution of states $D$ (e.g. distribution of users or documents we have to summarize).

Our task consists in learning to construct good lists of pre-specified length $k$ under some unknown
distribution of states $D$ (e.g. distribution of users or documents we have to
summarize). We consider two cases: context-free and contextual.
%\vspace{-0.1in}
%\begin{enumerate}
%\item The context-free case where we have no information about the current state of the world (e.g. we do not know
%anything about the user who is viewing the website)
%\item The contextual case where we observe some features of the state $x$ before choosing the list of
%items. 
%\end{enumerate}
%\vspace{-0.1in}


\textbf{Context-Free.}
In the context-free case, we have no side-information about the current state (i.e. we do not observe anything about $x$).  We quantify the performance of any list $L$ by its expected value:
$$F(L) = \mathbb{E}_{x  \sim D}[f_x(L)].$$
Note that $F(L)$ is also monotone submodular. Thus the clairvoyant greedy
algorithm with perfect knowledge of $D$ can find a list $\hat{L}_k$ such that $F(\hat{L}_k) \geq
(1-1/e) F(L^*_k)$, were $L^*_k = \argmax_{L:|L|=k} F(L)$. 
Although $D$ is unknown, we assume that we observe
samples of the objective $f_x$ during training.  Our goal is thus to develop a learning approach that efficiently converges, both computationally and statistically, to the performance of the clairvoyant greedy algorithm.% \todo{YY: reworded this to semantically match the modified introduction.}
%and would like to achieve a similar guarantee
%to the greedy algorithm in the limit as we observe more and more data.

%\todo{It it not necessary that we observe all of $x$-- i.e. the function can still appear stochastic even given $x$. How should we change that?}

\textbf{Contextual.}
In the contextual case, we observe side-information in the form of features regarding the state of the world.  We ``lift''  this problem to a hypothesis space of policies  (\emph{i.e.} multi-class predictors) that map
%we consider a ``lifting'' of the problem to a
%hypothesis space of policies (essentially multi-class predictors) that map
features to items. 

Let $\Pi$ denote our policy class, and let $\pi(x)$ denote the prediction of policy $\pi \in \Pi$ given side-information describing state $x$.
%the item chosen by a policy in that class in state $x$ as $\pi(x)$. 
Let $L_{\pi,k} = (\pi_1,\pi_2,\dots,\pi_k)$ denote a list of policies. In state $x$, this list of policies will predict 
$L_{\pi,k}(x) = (\pi_1(x),\pi_2(x),\dots,\pi_k(x))$. We quantify performance using the expected value:
$$F(L_{\pi}) = \mathbb{E}_{x \sim  D}[f_x(L_\pi(x))].$$ 
%$F$ can be seen as a list function, where items
%are policies $\pi \in \Pi$, and it can be seen that this lifted function
It can be shown that $F$ obeys both monotonicity and submodularity with respect to appending policies \cite{deyConSeqOptRSS}. Thus, a clairvoyant
greedy algorithm that sequentially picks the \emph{policy} with highest expected benefit
will construct a list $\hat{L}_{\pi,k}$ such that
$F(\hat{L}_{\pi,k}) \geq (1-1/e) F(L^*_{\pi,k})$, where $L^*_{\pi,k} = \argmax_{L_{\pi}:|L_{\pi}| = k} F(L_{\pi})$.
As before, our goal is to develop a learning approach (for learning a list of policies) that \emph{efficiently} competes with the performance of the clairvoyant greedy algorithm.% 
%Note that the oracle submodular function cannot be queried at prediction time. 

%\subsection{Reduction to Online Learning}

\subsection{The online learning approach}
\subsubsection{The Locally Greedy Regret}

\subsection{Submodular Contexual Policy Algorithm}
%\subsection{Extension for Knapsack Constraint}
%\subsection{Matroid Constraint}
\section{The imitation learning approach}


\section{Contextual Greedy Algorithm Unconstrained Submodular Maximization}
\subsection{Exact Maximization for Modular Function}
\subsection{Near Optimal Bi-directional Greedy}

==> outerLoopSCP1_flat.tex <==
We begin by defining a natural scoring function to evaluate any input list of chunks given ground-truth on the pixels corresponding to objects of interest in a scene. We provide an efficient greedy algorithm that is guaranteed to optimize this metric to within a constant factor given access to ground ground truth and this arbitrary list of (potentially overlapping) candidate chunks (Section \ref{sec:list_gt}). 

Of course, at testing time there is no access to the ground truth of where objects are in the scene. Our approach then, following recent work in structured prediction \cite{ross2013learning, daume2009search}, is to learn to mimic the sequential greedy strategy. The result is a simple predictor that takes a candidate set of chunks, and iteratively grows a list of chunks that likely correspond to separate objects in the scene.

Note that we do not place assumption on the given candidate set of chunks: the list predictor is agnostic to the way the candidate set of chunks was generated; it merely chooses the best one  in the set. Such a set can be heuristically generated in many ways, \emph{e.g.}, those created from the baseline approaches to visual chunking we describe above. In section \ref{sec:chunk_grow}, however, we provide an algorithm designed to generate a candidate set that contains good chunks based on a fixed superpixel-based segmentation.

\subsubsection{Objective Function and Greedy Optimization} \label{sec:list_gt}
Given an image with ground truth entities set $G$ and candidate chunks set $C$, our goal is to sequentially build a list of chunks out of $C$ so as to maximize the sum of intersection over union with respect to ground truth entities. Define $L = \{c_1, c_2, \dots, c_{|L|} \}$ as a list of chunks with $c_i \in C$, and $\tilde{G} = \{ \tilde{g}_1, \tilde{g}_2, \dots, \tilde{g}_{|L|}  \}$ with $\tilde{g}_i$ either an element from $G$ or a ``dummy" ground truth entity which gives zero I/U score. 

Each $c_i$ is associated with exactly one $\tilde{g}_i$, and each $\tilde{g}_i$ is associated with at most one $c_i$ (usually exactly one, unless we have less chunks than ground truth entities). Chunks that do not overlap ground truth objects have zero score. ``Dummy" ground truth is used as a notational convenience, to handle cases when the length of predicted list is larger the total number of ground truth entities, where some chunks in $L$ would otherwise have no ground truth entity to associate with. 
For any given list $L$ and $\tilde{G}$, let $h(L, \tilde{G})$ be the sum of I/U sores of the corresponding associations:
\begin{equation*}
    h(L, \tilde{G}) = \sum_{i=1}^{|L|}\|\frac{c_i\cap{\tilde{g}_i}}{c_i\cup{\tilde{g}_i}} \|
\end{equation*}
We define the score of the list, $f(L)$, to be the sum of I/U scores for the optimum association with ground truth entities, i.e., $f(L) = \{\max_{\tilde{G}} h(L, \tilde{G}) \} $.   We can express our goal in terms of maximizing the following objective function $f$:
\begin{equation}
	 \max_{L} f(L) = \max_{L}\{\max_{\tilde{G}} \sum_{i=1}^{|L|} \frac{\|c_i\cap{\tilde{g}_i}\|}{\|c_i\cup{\tilde{g}_i\|}} \} \label{list_obj_func} .
\end{equation}
%$f(L) = \{\max_{\tilde{G}} \sum_{i=1}^m \frac{c_i\cap{\tilde{g}_i}}{c_i\cup{\tilde{g}_i}} \} $ is the sum of intersection over union of each chunk-ground truth entity association over the best permutation $\tilde{G}$.  
This scoring metric, which is a natural generalization of the Intersection over Union metric common in segmentation and single entity detection \cite{Everingham10, arbelaez2012semantic}, encourages 
lists of a fixed length that contain chunks that are relevant and diverse in covering multiple ground truth entities. 
Unfortunately, the metric as written down does not possess the clear combinatorial structure like modularity or submodularity 
that would enable us to easily optimize it.

Interestingly, however, Problem~(\ref{list_obj_func}) can be cast as an equivalent maximum weighted bi-partite graph matching problem. This can be shown to be a  simple modular (i.e. additive) maximization problem under matroid constraints~\cite{lin2011word} and the solution $L^{gr}$ returned by a simple greedy algorithm is guaranteed to be near-optimal~\cite{fisher1978analysis}. The greedy algorithm then constructs a list $L^{gr}$ using the corresponding $\tilde{G}^{gr}$ as follows:
\begin{align*}
(c_{1}^{gr}, \tilde{g}_{1}^{gr})  & =  \argmax_{c \in C, g\in G}\frac{\|c \cap g\|}{\|c \cup g\|}, \\ 
 (c_{2}^{gr}, \tilde{g}_{2}^{gr}) & =  \argmax_{c \in C \setminus{c_1^{gr}}, g \in G \setminus{\tilde{g}_{1}^{gr}} }\frac{\|c \cap g\|}{\|c \cup g\|},  \\
 \vdots\\
 (c_{k}^{gr}, \tilde{g}_{k}^{gr}) & =  \argmax_{c\in C \setminus {\{c_1^{gr} \dots c_{k-1}^{gr}\}}, g \in G \setminus {\{\tilde{g}_1^{gr} \dots \tilde{g}_{k-1}^{gr}\}}}\frac{\|c \cap g\|}{\|c \cup g\|} 
\end{align*}

Critically, the greedy algorithm is recursive, meaning longer lists of predictions always include shorter lists, and is within a constant factor of optimal:
\begin{thmNearOptGreedyDef}
Let $L_{i}^{gr}$, $ \tilde{G}_{i}^{gr}$ denote the list of the first $i$ elements in $L^{gr}$ and $\tilde{G}^{gr}$ respectively, and $L_{i}^*$ be the optimal solution of Problem (\ref{list_obj_func}) among size-$i$ lists, we have that:
\begin{displaymath}  
f(L_{i}^{gr}) \geq h(L_{i}^{gr}, \tilde{G}_{i}^{gr}) \geq \frac{1}{3} f(L_{i}^*)
\end{displaymath}
for $i = 1,...,|L^{gr}|$.
\end{thmNearOptGreedyDef}
%See appendix for proof of Theorem \thmNearOptGreedy. 
The implication of Theorem \thmNearOptGreedy is that if we are given a budget $|L|$ to build the list, then each $L_{i}^{gr}$ is also a near optimal list among all lists of budget $i$, for $i=1, \dots, |L|$. This is an important property for producing good predictions earlier in the list and for producing the list of chunks rapidly.
Moreover, this is the worst case bound, and in our empirical experiments, the quality of solutions are usually much better than this bound suggests. 

\subsubsection{List Prediction Learning} \label{sec:list_learning}
In essence, the greedy strategy is a sequential list prediction process, where at each round, it maximizes the marginal benefit given the previous list of predictions and ground truth association. Intuitively, maximization of the marginal benefit at each position of the list yields chunks that have high intersection over union with ground truth entities and minimal overlap with each other. 

%We would like to train a predictor to imitate the above sequential greedy process. To be concrete, at each round $r$, the predictor should rank each of unassigned candidate chunk $c$ based on a score $h(c) = \max_{g \in G_{re}} \frac{c \cap g}{c \cup g}$, where $G_{re}$ is the remaining  ground truth entities.

We adopt an approach following that of \cite{ross2013learning, ross2011learning} where we train a learning algorithm to mimic this greedy procedure. The  training procedure as illustrated in Algorithm \ref{outerloop_training}.  We denote by $\Phi(c, L)$ the feature vector that represents the interaction between each input chunk $c$, any given list $L$ and their interactions. This includes features measuring the affinity or similarity between $c$ and elements in $L$, and intuitively, a high affinity feature implies that appending $c$ to $L$ is less preferred as it is similar to exising items in the list. We discuss the features design in \ref{sec:features}.
We denote $\tilde{G}^{gr}(L)$  the corresponding greedy association for any list $L$,  we define the greedy marginal benefit of adding chunk $c$ to $L$ be $y(c, L) = h(L\oplus c, \tilde{G}^{gr}(L\oplus c)) - h(L, \tilde{G}^{gr}(L)) $.

\begin{algorithm}[!t] 
\caption{List Predictor Training Algorithm Using DAgger}
\label{outerloop_training}
\begin{algorithmic}
\STATE \textbf{Input:}  $T$ images, each with candidate chunk set $C^t$ and $G^t$, number of training iterations $R$, list size $k$  
\STATE \textbf{Output:} A trained list predictor/predictor $\pi$
\STATE Initialize $D \gets \emptyset$
\STATE Set $\pi_0$ to be the greedy oracle predictor 
\FOR{$i = 1$ \textbf{to} $R$ }
	\FOR{$t = 1$ \textbf{to} $T$}
	\STATE $L^t = $\textrm{Predict}$(C^t, \pi_{i-1}, k)$.
	\STATE Get dataset $D^t_i = \{ X_{j=1}^{k}, Y_{j=1}^{k} \}$ using $L^t$, $C^t$ and $G^t$.
	\STATE $D \gets D \cup D^t_i$.
	\ENDFOR
	\STATE Train $\pi_{i}$ on D
\ENDFOR
\STATE Return $\pi_{R}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!t] 
\SetAlgorithmName{Procedure}{procedure}{List of procedure}
%\caption{Predict$(C, \pi_{i-1}, k)$}
%\begin{small}
\begin{algorithmic}
\STATE \textbf{Procedure:} Predict$(C, \pi_{i-1}, k)$ 
\STATE \textbf{Input:} Candidate chunk set $C$, List Predictor $\pi$, list size $k$ 
\STATE \textbf{Output:} A list $L$ of chunks
\STATE Initialize $L$ = \{ \}.
\FOR{$ i = 1$ \textbf{to} $k$}
	\STATE $c_i = \argmax_{c \in C}\pi(\Phi(c, L ))$
	\STATE $L = L \oplus c_i$
\ENDFOR
\STATE Return L
\end{algorithmic}
%\end{small}
\end{algorithm}

   The DAgger training mechanism is beneficial in that the policy iteration collects data aimed to improve its own performance. See \cite{ross2010reduction} for more details.  
  %This training algorithm is iterative and begins by generating data assuming all earlier positions in the list were filled in using the greedy predictor with oracle access to the ground truth data. After the first iteration, however, it is learning to correct it's own mistakes: i.e. it will learn that earlier predictions maybe imperfect and adjust the lists it creates.
  
  In each iteration, the predictor from last iteration loops over every training image $t$ and generates a list prediction $L^t$, as illustrated in $\mathrm{Predict()}$ procedure. As this list is built, we record the marginal benefit of adding other possible elements. Consider the case where the predictor initially chooses a chunk that covers the entire image, in which there is a single ground truth entity. We can improve the list by appending to it a chunk that has a higher I/U score with the entity, and then updating the association between chunks and entities
 
The algorithm then collects target data $D^t_i = \{ X_{j=1}^{k}, Y_{j=1}^{k} \}$ consisting of features and the true marginal benefits measure on training data using $L^t$, $C^t$ and $G^t$, where: 
	\begin{enumerate}
	\item $ X_{j=1}^{k}$ is a collection of feature matrices whose element $X_j$ of size $|C_t| \times d$ is formed by stacking the $d$-dimenional feature vectors $\Phi(c, L_j)$, where $c\in C^t$ and $L_j$ is the list of the first $j$ elements in $L$
	\item $Y_{j=1}^k$  is a collection of greedy marginal benefit vectors whose  element $Y_j$ of length $|C_t|$ records $y(c, L_j)$ for each chunk $c\in C^t$
	\end{enumerate}
Each $D^t_i$ is appended to the old training data collection from last iteration to form a larger training dataset $D$, before being utilized to train a regression that predicts benefits. 

Given a new image with a set of candidate chunks, we can call  $\mathrm{Predict()}$ procedure to produce a list of specified length. 


==> results_flat.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
test change

We evaluate our approach on the Stanford Background Dataset \cite{gould2009decomposing}, and additionally relabled it to separate 'vehicles' and 'person' from the original, broader, 'foreground' category.  

  


%% We also used a dataset culled from public Flickr data, consisting of arid urban and suburban scenes, some of which contain vehicles and people. The class set of this dataset (``Desert Flickr'') is more diverse than that of the Stanford Background Dataset (SBD), and thus performance degrades.  

%% \tiny
%% \begin{table*}
%% \scriptsize
%% \begin{adjustwidth}{-10mm}{}

%% \centering
%% \caption{Improving Semantic Segmentation with Object Detectors} \label{tab:ss_improvement1}

%% \begin{tabular}{|l|c|c||c|c||c|c||c|c||}
%% \cline{1-9}
%% & SBD 8 & SBD 8 w/ Detectors & SBD 13 & SBD 13 w/ Detectors & Desert Flickr & Desert Flickr w/ Detectors & DFSBD & DFSBD w/ Detectors\\
%% \hline
%% Per-class Mean Precision & 71.91 & 72.57 & 62.50 & 63.34 & 27.80 & 33.21 & 27.78 & 25.89 \\
%% \hline
%% Per-class Mean Recall & 69.17 & 69.92 & 56.72 & 57.14 & 23.14 & 24.13 & 22.41 & 21.23  \\
%% \hline
%% Per-class Accuracy & 58.41 & 59.40 & 44.19 & 45.04  & 17.30 & 18.18 & 16.67 & 15.69\\
%% \hline
%% Vehicle F1 & \footnotemark[1] & \footnotemark[1] & 70.07 & \textbf{74.58}  & 31.12 & \textbf{42.42} & 24.29 & \textbf{42.13}\\
%% \hline
%% Person F1 & \footnotemark[1] & \footnotemark[1] & 50.58 & \textbf{55.69}  & 72.54 & \textbf{74.15} & 72.12 & \textbf{74.27} \\
%% \hline
%% Overall Accuracy & 80.93 & 81.64 & 72.21 & 73.26 & 61.02 & 63.06 & 62.52 & 63.18 \\ 
%% \hline
%% \end{tabular} \\

%% %% \vspace{5mm}
%% %% \centering
%% %% \begin{tabular}{|l|c|c||c|c|}
%% %% \cline{1-5}
%% %% & Desert Flickr & Desert Flickr w/ Detectors & DFSBD & DFSBD w/ Detectors \\
%% %% \hline
%% %% Per-class Mean Precision & 27.80 & 33.21 & 27.78 & 25.89 \\
%% %% \hline
%% %% Per-class Mean Recall & 23.14 & 24.13 & 22.41 & 21.23 \\
%% %% \hline
%% %% Per-class Accuracy & 17.30 & 18.18 & 16.67 & 15.69 \\
%% %% \hline
%% %% Vehicle F1 & 31.12 & \textbf{42.42} & 24.29 & \textbf{42.13} \\
%% %% \hline
%% %% Person F1 & 72.54 & \textbf{74.15} & 72.12 & \textbf{74.27} \\
%% %% \hline
%% %% Overall Accuracy & 61.02 & 63.06 & 62.52 & 63.18 \\ 
%% %% \hline
%% %% \end{tabular}
%% \footnotemark[1] SBD Datset has no 'vehicle' or 'person' classes.
%% \end{adjustwidth}
%% \end{table*}
%% \normalsize
%% \FloatBarrier


%% \subsection{Semantic Segmentation}

%% The results of improving semantic segmentation by incorporating object detectors as features are shown in Table \ref{tab:ss_improvement1}. Most performance gains were in the individual class relevant to the detector, however, gains in overall performance and the performance of other classes manifested as well.



%% \subsection{Refining Object Detection}
%% The results of improving vehicle and face detection are shown in Table \ref{tab:pr_context_improvement1} and Figure \ref{fig:edr1}. As explained in Section \ref{sec:approach_refining_detections}, this approach is intended to enhance the precision of an object detector. Improving detectors with very low precision yields significant gains in precision. In the most extreme case, the person detector precision was improved from less than 1\% to approximately 22\% precision, with negligible decline in recall.

%% \tiny

%% \begin{table*}
%% \begin{center}
%% \caption{Performance of object detectors with and without context, computed across 5 SBD folds} \label{tab:pr_context_improvement1}
%% \begin{tabular}{|l||c|c|c||c|c|c|}
%% \cline{1-7}
%%   & Vehicle & Vehicle with Context & Improvement  & Person  & Person with Context & Improvement \\
%% \hline
%% Max Recall & \textbf{.19 $\pm$ .01} & .18 $\pm$ .02 & -5.3\% & \textbf{.31 $\pm$ .04} & .29 $\pm$ .05 & -6.5\%  \\
%%   Precision\footnotemark[2] & .066 $\pm$ .008 & \textbf{.16 $\pm$ .02} & 150\% & .0066 $\pm$ .0008  & \textbf{.22 $\pm$ .03} & 3,200\%\\  
%% \hline
%% \hline
%%   \textbf{Max F1}  & .154 $\pm$ .009 & \textbf{.21 $\pm$ .02} & 36\% & .16 $\pm$ .01 & \textbf{.21 $\pm$ .02} & 31\%\\ 
%% \cline{1-7}
%% \end{tabular}

%% \vspace{5pt}

%% \end{center}
%% \footnotemark[2]\footnotesize Precision corresponding to Max Recall
%% \end{table*}

%% \normalsize

%% %      P3norm recall      P3inf  recall   P3normprecision  P3inf precision      P3norm F1    P3inf F1
%% % f0      .33152       .31636              .00718              .24178             .1533         .2071
%% % f1       .30851        .29453            .006291             .22872             .1494         .2243
%% % f2      .29231       .26831             .006228             .21272              .1560          .2317
%% % f3       .36735         .34408            .007643            .25762             .1439          .1796
%% % f4     .26738    .21992                  .005635             .18118             .1796          .2171
    


%% \newlength{\colsquish}
%% \setlength{\colsquish}{-26pt}
%% \newlength{\graphwidth}
%% \setlength{\graphwidth}{.43\textwidth}

%% \begin{figure*}
%% \caption{Performance of Detectors With and Without Context across 5 SBD folds} \label{fig:edr1}
%% \begin{subfigure}[b]{\textwidth}
%% \centering
%% \includegraphics[width=.8\textwidth]{img/Original_vs_Context-Aware_Performance_of_Person_and_Vehicle_Detectors.png} 
%% \end{subfigure}
%% \end{figure*}

%% \begin{figure*}[t]
%% \caption{Precision vs. Recall of Standard and Context-Aware Vehicle Detections} \label{fig:edr1}

%% \begin{subfigure}[b]{1.3\textwidth}
%% \hspace{-60pt} \includegraphics[width=\graphwidth]{img/SBD_vehicle_0.png} \hspace{\colsquish} \includegraphics[width=\graphwidth]{img/SBD_vehicle_1.png} \hspace{\colsquish} \includegraphics[width=\graphwidth]{img/SBD_vehicle_2.png} \\
%%  \hspace{30pt} \includegraphics[width=\graphwidth]{img/SBD_vehicle_3.png} \hspace{\colsquish} \includegraphics[width=\graphwidth]{img/SBD_vehicle_4.png}
%% \end{subfigure}


%% \end{figure*}

%% \begin{figure*}[t] 
%% \caption{Precision vs. Recall of Standard and Context-Aware Person Detections} \label{fig:edr1}
%% \centering

%% \begin{subfigure}[b]{1.3\textwidth}
%% \hspace{-60pt} \includegraphics[width=\graphwidth]{img/SBD_person3_0.png} \hspace{\colsquish} \includegraphics[width=\graphwidth]{img/SBD_person3_1.png} \hspace{\colsquish} \includegraphics[width=\graphwidth]{img/SBD_person3_2.png} \\
%% \hspace{80pt} \includegraphics[width=\graphwidth]{img/SBD_person3_3.png} \hspace{\colsquish} \includegraphics[width=\graphwidth]{img/SBD_person3_4.png}
%% \end{subfigure}


%% \end{figure*}



%\clearpage


==> subModFunc_local_conflict_flat.tex <==
  


==> submodFunc_flat.tex <==
Given an image with ground truth entities $G = \{g_1, g_2, \dots, g_k\}$ and candidate chunks set $C = \{c_1, c_2, \dots, c_n \}$, our goal is to select the optimal $k$ chunks out of $C$ and associate each with the ground truth entities so as to maximize the sum of intersection over union scores for each association. This is a classic assignment problem in combinatorial optimization, which is equivalent to computing the maximum weighted bi-partite graph matching. The edge set $E$ of the bi-partite graph is the Cartesian product of $G$ and $C$, i.e., $E = G \times C$. The weight $w_{ij}$ for each edge $e_{ij}$ is assigned as the I/U score of chunk $c_i$ and ground truth $g_j$. 
We now express bi-partite matching as intersection of two partition matroids. A matroid is a structure that generalize the linear independence in vector spaces. A matroid is a pair $(E, \mathcal{I})$, where $E$ is the ground set and $I$ is a collection of independent subsets of $E$, that satisfies: (\rmnum{1}) \textit{hereditary property}: for each $A' \subset A \subset E$, if $A \in \mathcal{I} $ then $A' \in I $, and (\rmnum{2}) \textit{augmentation property}: if $A, B \in E$ and $|A| < |B|$, then there exists some element $e\in B\setminus A$ such that $A\cup{e} \in I$.  

 Let $E_{i}^G = G \times \{i\}$ be all the edges that connect to $c_i$ and $E_{j}^C = \{j\} \times C$ be all the edges that connect to $g_j$. $\{ E_{i}^G : i\in C \}$ and $\{ E_{j}^C : j\in G \}$ are partitions of the ground set $E$, inducing two 1-partition matroids $(E, \mathcal{I}_C)$:
\begin{align*}
\mathcal{I}_C  =  \{ A \subseteq E:  \forall g_j \in G, |A \cap E_{j}^C| \leq 1 \},  \\
\mathcal{I}_G  =  \{ A \subseteq E:  \forall c_i \in C, |A \cap E_{i}^G| \leq 1 \} 
\end{align*}  
Therefore we can formulated the problem as below:
\begin{equation}
\max_{A\subseteq E} f(A), \text{subject to } A \in I = I_C \cap I_G
\label{modular_max_matroid}
\end{equation} 
, where $f$ is a modular (and hence submodular) function defined as the sum of the weights of $A$. Hungarian algorithm (or Kuhn-Munkres algorithm)[CITE KM] runs in $\BigO{n^3}$ time to compute the optimum solution for \ref{modular_max_matroid}. However, from the learning perspective, it's hard to imitate the algorithmic procedure of Hungarian algorithm. It turns out that a simple greedy algorithm with empty set initialization\cite{fisher1978analysis}, as shown in \ref{greedy_modular_matroid}, is guaranteed to satisfy that $f(A_g) \geq \frac{1}{m+1}\max_{A \in I}f(A)$, where $I = \bigcap_{i=1}^m I_i$ is the intersection of all independent sets. In this case, $m=2$ and therefore $f(A_g) \geq \frac{1}{3}f(A*)$. Note that this is the worst case bound, and in our empirical experiments, the quality of solution is usually much better than this bound suggests. 
\begin{equation} 
A_g \gets A_g \cup \{ \argmax_{e \notin A_g: A_g\cup{e}\in\mathcal{I}} \Delta(e|A_g) \}
\label{greedy_modular_matroid}
\end{equation}
Note that the greedy algorithm in \ref{greedy_modular_matroid} is selecting candidate chunks sequentially, denote the output list of chunks be $L$, then we have $L = \{c_{i_1}, c_{i_2}, ... , c_{i_k}\}$, where:
\begin{align*}
(c_{i_1}, g_{i_1})  & =  \argmax_{c \in C, g\in G}\frac{c \cap g}{c \cup g}, \\ 
 (c_{i_2}, g_{i_2}) & =  \argmax_{c \in C \setminus{c_{i_1}}, g \in G \setminus{g_{i_1}} }\frac{c \cap g}{c \cup g},  \\
 \vdots\\
 (c_{i_k}, g_{i_k}) & =  \argmax_{c\in C \setminus {\{c_1 \dots c_{k-1}\}}, g \in G \setminus {\{g_1 \dots g_{k-1}\}}}\frac{c \cap g}{c \cup g} 
\end{align*}

\begin{comment}
suppose the algorithm output a set of predicted chunks $C = \{c_1, c_2, \dots , c_k\}$ we would like to evaluate the performance of $C$. 
Let $\{c_{i_1}, c_{i_2}, \dots, c_{i_k}\}$ and $\{g_{i_1}, g_{i_2}, \dots, g_{i_k}\}$ be two sequences such that:
\begin{align*}
(c_{i_1}, g_{i_1}) & = & \argmax_{c \in C, g\in G}\frac{c \cap g}{c \cup g}, \\ 
 (c_{i_2}, g_{i_2}) & = & \argmax_{c \in C \setminus{c_{i_1}}, g \in G \setminus{g_{i_1}} }\frac{c \cap g}{c \cup g},  \\
 \vdots\\
 (c_{i_k}, g_{i_k}) & = & \argmax_{c\in C \setminus {\{c_1 \dots c_{k-1}\}}, g \in G \setminus {\{g_1 \dots g_{k-1}\}}}\frac{c \cap g}{c \cup g} 
\end{align*}
The objective function is defined as sum of intersection over union follows: 
\begin{equation}
f(C;G) = \sum_{s=1}^{k} \frac{c_{i_{s}} \cap g_{i_{s}}}{c_{i_{s}} \cup g_{i_{s}}}, \\ 
\label{eq:sumIOverU}
\end{equation}
It can be easily seen that the objective function $f$ is submodular since the intersection term 
We are interested optimizing the average 
\end{comment}

==> temp2_flat.tex <==

\begin{algorithm}

\begin{algorithmic}
\State Input: Data

\end{algorithmic}
\end{algorithm}


==> us_vs_them_flat.tex <==
\newlength{\expImgLen}
\setlength{\expImgLen}{.1\textwidth}

%% \begin{figure}[t!]
%% \centering
%% \begin{subfigure}{\textwidth}
%% \centering
%% \includegraphics[width=.24\textwidth]{img/us_vs_them/0100628_dpm_crop.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/0100628_1overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/0100628_2overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/0100628_3overlayed.png}\\
%% \vspace{2pt}

%% \vspace{2pt}
%% \includegraphics[width=.24\textwidth]{img/us_vs_them/1001770_dpm_crop.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1001770_1overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1001770_2overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1001770_3overlayed.png}\\
%% \includegraphics[width=.24\textwidth]{img/us_vs_them/6000197_dpm_crop.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/6000197_1overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/6000197_2overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/6000197_3overlayed.png}\\
%% \includegraphics[width=.24\textwidth]{img/us_vs_them/1000288_dpm.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1000288_1overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1000288_2overlayed.png}\\
%% \end{subfigure}
%% \caption{Comparison between our system and the DPM baseline. The leftmost images are the top 3 DPM detections. Other images are from our system. The first prediction is shown in red, the second prediction is shown in green, and the third in blue.} \label{fig:us_vs_them}
%% \hfill
%% \end{figure}

%\begin{figure}[t!]
%\centering
%\begin{subfigure}%{textwidth}

%\includegraphics[width=\expImgLen]{img/us_vs_them/0100628_dpm_crop.png} \includegraphics[width=\expImgLen]{img/us_vs_them/0100628_1overlayed.png} \includegraphics[width=\expImgLen]{img/us_vs_them/0100628_2overlayed.png} \includegraphics[width=\expImgLen]{img/us_vs_them/0100628_3overlayed.png}\\
%\vspace{2pt}

%% \vspace{2pt}
%% \includegraphics[width=.24\textwidth]{img/us_vs_them/1001770_dpm_crop.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1001770_1overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1001770_2overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1001770_3overlayed.png}\\
%% \includegraphics[width=.24\textwidth]{img/us_vs_them/6000197_dpm_crop.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/6000197_1overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/6000197_2overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/6000197_3overlayed.png}\\
%% \includegraphics[width=.24\textwidth]{img/us_vs_them/1000288_dpm.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1000288_1overlayed.png} \includegraphics[width=.24\textwidth]{img/us_vs_them/1000288_2overlayed.png}\\


%\end{subfigure}
%\caption{Comparison between our system and the DPM baseline. The leftmost images are the top 3 DPM detections. Other images are from our system. The first prediction is shown in red, the second prediction is shown in green, and the third in blue.} \label{fig:us_vs_them}
%\hfill
%\end{figure}

